Are We Learning the Right Features? A Framework for Evaluating DL-Based Software Vulnerability Detection Solutions

Recent research has revealed that the reported results of an emerging body of DL-based techniques for detecting software vulnerabilities are not reproducible, either across different datasets or on unseen samples. This paper aims to provide the foundation for properly evaluating the research in this domain. We do so by analyzing prior work and existing vulnerability datasets for the syntactic and semantic features of code that contribute to vulnerability, as well as features that falsely correlate with vulnerability. We provide a novel, uniform representation to capture both sets of features, and use this representation to detect the presence of both vulnerability and spurious features in code. To this end, we design two types of code perturbations: feature preserving perturbations (FPP) ensure that the vulnerability feature remains in a given code sample, while feature eliminating perturbations (FEP) eliminate the feature from the code sample. These perturbations aim to measure the influence of spurious and vulnerability features on the predictions of a given vulnerability detection solution. To evaluate how the two classes of perturbations influence predictions, we conducted a large-scale empirical study on five state-of-the-art DL-based vulnerability detectors. Our study shows that, for vulnerability features, only ~2% of FPPs yield the undesirable effect of a prediction changing among the five detectors on average. However, on average, ~84% of FEPs yield the undesirable effect of retaining the vulnerability predictions. For spurious features, we observed that FPPs yielded a drop in recall up to 29% for graph-based detectors. We present the reasons underlying these results and suggest strategies for improving DNN-based vulnerability detectors. We provide our perturbation-based evaluation framework as a public resource to enable independent future evaluation of vulnerability detectors.

==> cpg_rules/dealloc/double_free.tex <==

$\displaystyle F:$ Set of library functions used for allocating heap memory.\\

$\displaystyle V':$ Set of CPG nodes calling any function $\displaystyle f\in F$\\

$\displaystyle V':=\{ v\in V:\mu ( v,K=``type") =``CallExpression"\ \land \mu ( v,K=``Callee") \in F\ \}$\\

\textbf{Rule 2.6: }$\displaystyle \exists v\in V':\exists x\in DA_{b} :\exists y\in DA_{b} ,( edge( x,y) \in E) \land ( \lambda ( x,y) =``POST\_DOM") \land ( \forall z\in A_{b} ,\ ( edge( x,z) \notin E\lor \lambda ( x,z) \neq ``POST\_DOM")$; Where,\\
$\displaystyle b:$ allocated buffer variable in node $\displaystyle v$\\
$\displaystyle A_{b} :$ CPG Nodes performing allocation operation for buffer $\displaystyle b$\\
$\displaystyle DA_{b} :$ CPG Nodes performing deallocation operation for $\displaystyle b$
\begin{gather*}
b:=\mu ( v,K=``dest\_identifier")\\
A_{b} :=\{z\in V':\mu ( z,K=``dest\_identifier") =b\}\\
DA_{b} :=\{u\in V:edge( v,\ u) \in E \\
\land \lambda ( v,u) =``REACHES"\land \mu (( v,u) ,K=``var") =b \\
\land \mu ( u,K=``type") =``CallExpression"\\
\land \mu ( u,K=``Callee") =``free"\}
\end{gather*}

==> cpg_rules/dealloc/use_after_free.tex <==

\textbf{Rule 2.7: }$\displaystyle \exists v\in V':\exists x\in RD_{b}:\exists y\in DA_{b} ,( edge( x,y) \in E) \land ( \lambda ( x,y) =``POST\_DOM") \land ( \forall z\in A_{b} ,\ ( edge( x,z) \notin E\lor \lambda ( x,z) \neq ``POST\_DOM")$; Where,\\
$\displaystyle RD_{b} :$ Reaching Definitions for $\displaystyle b$\\

$\displaystyle RD_{b} :=\{\ u\in V:edge( v,\ u) \in E\ \land \lambda ( v,u) =``REACHES"\land \mu (( v,u) ,K=``var") =b\}$\\

==> cpg_rules/graph/edge_only.tex <==

$\displaystyle X_{1} ,X_{2} :$ Samples from the dataset.\\
% \saad{I think there is no need to mention SARD dataset as the rules are generic and can be applied to the code from any dataset.}

$\displaystyle E_{1} ,E_{2} :$ CPG edges of the samples $\displaystyle X_{1} \&X_{2}$.\\

$\displaystyle Y_{1} ,Y_{2} :$ Line level ground truth containing the set of vulnerable lines in the samples $\displaystyle X_{1} \&X_{2}$.\\

\textbf{Rule 2.11: } $\displaystyle \exists ( u,v) \in E_{1}:( u,v) \in E_{2} \land ( u\in Y_{1} \lor v\in Y_{1}) \land ( u\notin Y_{2} \land v\notin Y_{2})$

==> cpg_rules/graph/node_only.tex <==

$\displaystyle V_{1} ,V_{2} :$ Sets of CPG nodes for the samples $\displaystyle X_{1} \&X_{2}$.\\

$\displaystyle \mu _{1} ,\ \mu _{2} :$ CPG property functions for the samples $\displaystyle X_{1} \&X_{2}$.\\

$\displaystyle V_{1} ':$ CPG nodes for the sample $\displaystyle X_{1}$ that are vulnerable in sample $\displaystyle X_{1}$ but benign in $\displaystyle X_{2}$.\\

\textbf{Rule 2.12: } $\displaystyle V_{1} '\neq \phi $; Where,\\

$\displaystyle V_{1} ':=\{v\in V_{1}:v\in V_{2} \land ( \mu _{1}( v,K=``loc") \in Y_{1} \land \mu _{2}( v,K=``loc") \notin Y_{2})\}$\\

==> cpg_rules/num_range/underread.tex <==

$\displaystyle V_{r} ':$ Set of CPG nodes reading from buffer $\displaystyle b$ using an index variable\\

$\displaystyle idx:$ Index used in node $\displaystyle v \in V_{r} '$\\

$\displaystyle C_{idx}^{v} :$ Control nodes for node $\displaystyle v$ checking numeric comparison between $\displaystyle idx$ and $\displaystyle 0$\\

$\displaystyle V_{r} ':=\{v\in V':\exists u\in V,\ edge( v,u) \in E\land \lambda ( v,u) =``USE"\land \mu ( u,K=``Symbol") =b\}$\\

\textbf{Rule 2.9: } $\displaystyle C_{idx}^{v} =\phi $\\

==> cpg_rules/num_range/underwrite.tex <==

$\displaystyle V':$ Set of CPG nodes containing a buffer access using an index\\

$\displaystyle b:$ Buffer used in node $\displaystyle v \in V '$\\

$\displaystyle V_{w} ':$ Set of CPG nodes writing to buffer $\displaystyle b$ using an index variable\\

$\displaystyle idx:$ Index used in node $\displaystyle v \in V_{w} '$\\

$\displaystyle C^{v} :$ Control nodes for node $\displaystyle v$ \\

$\displaystyle C_{idx}^{v} :$ Control nodes for node $\displaystyle v$ checking numeric comparison between $\displaystyle idx$ and $\displaystyle 0$\\

\begin{gather*}    
V':=\{v\in V:\mu ( v,K=``type") =``ArrayIndexing"\}\\
b,idx:=\mu ( v,K=``identifiers")\\
V_{w} ':=\{v\in V':\exists u\in V,\ edge( v,u) \in E\land \lambda ( v,u) =``DEF"\\
\land \mu ( u,K=``Symbol") =b\}\\
C^{v} :=\{u\in V:edge( u,v) \in E\land \lambda ( u,v) =``CONTROLS"\}\\
C_{idx}^{v} :=\{u\in C^{v} :\mu ( u,K=``type") =``RelationalExpression"\\
\land \mu ( u,K=``operator") =``\geqslant "\\
\land \mu ( u,K=``Identifier") =idx\\
\land \mu ( u,K=``PrimaryExpression") =0\}
\end{gather*}
\textbf{Rule 2.8: } $\displaystyle C_{idx}^{v} =\phi $\\

==> cpg_rules/overflow/heap_based.tex <==

$\displaystyle F_{1}:$ Set of library functions that write in buffers\\

$\displaystyle F_{2}:$ Set of library functions used for allocating heap memory\\

$\displaystyle V':$ Set of CPG nodes calling any function $\displaystyle f\in F_{1}$\\

$\displaystyle V':=\{ v\in V:\mu ( v,K=``type") =``CallExpression"\ \land \mu ( v,K=``Callee") \in F_{1}\ \}$\\

\textbf{Rule 2.5: }$\displaystyle \exists v\in V':( \exists u\in RD_{d} :\mu ( u,K=``type") =``CallExpression"\ \land \mu ( u,K=``Callee") \in F_{2})$; Where,\\
$\displaystyle d:$ Destination buffer in node $\displaystyle v$\\
$\displaystyle RD_{d} :$ Reaching Definitions for $\displaystyle d$\\

\begin{gather*}
d:=\mu ( v,K=``FirstArgument")\\
RD_{d} :=\{\ u\in V:edge( u,\ v) \in E\ \land \lambda ( u,v) =``REACHES"\\
\land \mu (( u,v) ,K=``var") =d\}\\
V':=\{ v\in V:\mu ( v,K=``type") =``CallExpression"\\\
\land \mu ( v,K=``Callee") \in F_{1}\ \}\\
\end{gather*}



==> cpg_rules/overflow/incorr_calc.tex <==

\textbf{Rule 2.1:}\\
\textbf{Data Segment:}\\
$\displaystyle F:$ Set of library functions that write in buffers\\
$\displaystyle V':$ Set of CPG nodes calling any function $\displaystyle f\in F$\\
$\displaystyle l:$ Length used in node $\displaystyle v$\\
$\displaystyle d:$ Destination buffer in node $\displaystyle v$\\
$\displaystyle s:$ Source buffer in node $\displaystyle v$\\
$\displaystyle L_{d}:$ Buffer lengths
% \saad{why is it lengths instead of length?}
for $\displaystyle d$\\
$\displaystyle L_{s}:$ Buffer lengths for $\displaystyle s$\\
\textbf{Traversal Segment:}\\
$\tau _{1} :V'=\{v\in V:\mu ( v,``type") =``CallExpression"\land \mu ( v,``Callee") \in F\}$\\
Query 2: $\displaystyle d,s,l\leftarrow \mu ( v,K:=``ArgumentList")$\\
Query 3: $\displaystyle L_{d}\leftarrow \{\mu ( u,K:=``use\_size") u\in V:u\rightarrow v\in E\land \lambda ( u,v) =``REACHES"\land \mu (( u,v) ,K:=``var") =d\}$\\
Query 4: $\displaystyle L_{s}\leftarrow \{\mu ( u,K:=``use\_size") u\in V:u\rightarrow v\in E\land \lambda ( u,v) =``REACHES"\land \mu (( u,v) ,K:=``var") =s\}$\\
\textbf{Condition Segment:}\\
$\displaystyle \exists v\in V':( l\notin L_{d}) \ \land ( l\notin L_{s}) \land ( \forall x\in L_{d} :x< l)$\\



% \textbf{Rule 2.1: }$\displaystyle \exists v\in V':( l\notin L_{d}) \ \land ( l\notin L_{s}) \land ( \forall x\in L_{d} :x< l)$; Where,\\

% \begin{gather*}
% d,s,l:=\mu ( v,K=``ArgumentList")\\
% L_{d} :=\{\mu ( u,K=``use\_size") \ u\in V:\\
% edge( u,\ v) \in E\ \land \lambda ( u,v) =``REACHES"\\
% \land \mu (( u,v) ,K=``var") =d\}\\
% L_{s} :=\{\mu ( u,K=``use\_size") \ u\in V:\\
% edge( u,\ v) \in E\ \land \lambda ( u,v) =``REACHES"\\
% \land \mu (( u,v) ,K=``var") =s\}
% \end{gather*}

==> cpg_rules/overflow/off-by-one.tex <==

\textbf{Rule 2.3: }$\displaystyle \exists v\in V':( l\notin L_{d}) \ \land ( l\in L_{s} ')$; Where,\\
$\displaystyle L_{s} ':$ Buffer lengths for $\displaystyle s$ that are greater than the length of $\displaystyle d$ by one.\\

$\displaystyle L_{s} ':=\{x\in L_{s} :\exists y\in L_{d} ,y+1=x\}$\\

==> cpg_rules/overflow/over_read.tex <==

\textbf{Rule 2.4: }$\displaystyle \exists v\in V':( l\notin L_{s}) \ \land ( l\in L_{d} ')$; Where,\\
$\displaystyle L_{d} ':$ Buffer lengths for $\displaystyle d$ that are greater than the length of $\displaystyle s$\\

$\displaystyle L_{d} ':=\{x\in L_{d} :\exists y\in L_{s} ,y< x\}$\\

==> cpg_rules/overflow/src_size.tex <==

\textbf{Rule 2.2: }$\displaystyle \exists v\in V':( l\notin L_{d}) \ \land ( l\in L_{s} ')$; Where,\\
$\displaystyle L_{s} ':$ Buffer lengths for $\displaystyle s$ that are greater than the length of $\displaystyle d$\\

$\displaystyle L_{s} ':=\{x\in L_{s} :\exists y\in L_{d} ,y< x\}$\\

==> cpg_rules/sensi_read_write/sensi_r_w.tex <==

$\displaystyle F:$ Set of library functions that read from or write in buffers.\\

$\displaystyle Y:$ Line level ground truth containing the set of vulnerable lines in the sample.\\

$\displaystyle \mathcal{L} :$ Set of code locations where there is a call to any function $\displaystyle f\in F$\\

\textbf{Rule 2.10: }$\displaystyle \mathcal{L} \cap Y\neq \phi $; Where,\\ 

$\displaystyle \mathcal{L} :=\{\mu ( v,K=``loc") \ v\in V:\mu ( v,K=``type") =``CallExpression"\ \land \mu ( v,K=``Callee") \in F\ \}$\\

==> detection_algorithms/dealloc/double_free.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwIn{$G=( V,E, \lambda, \mu )$ representing the CPG constructed from the sample code}
\KwOut{Boolean value indicating whether the feature exists in the sample\\
\textbf{Begin}}
Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = AF\}\;
\For{node $x$ in $V'$}
{
    Let $b$ $\gets$ $\mu(x, dest)$\;
    Let $DA_{b} \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = DF and $\mu(v, arg\_dest)=b$\}\;
    \For{node $v$ in $DA_{b}$}
    {
        \For{node $u$ in $DA_{b}$}
        {
            \uIf{$(u, v) \in E$ and $\lambda(u, v) = $ PD}
            {
                REALLOC\_FLAG $\gets$ $false$\;
                \For{node $w$ in $V'$}
                {
                    \uIf{$\mu(w, dest) = b$ and $(u, w) \in E$ and $\lambda(u, w) = $ PD and $(w, v) \in E$ and $\lambda(w, v) = $ PD}
                    {
                        REALLOC\_FLAG $\gets$ $true$\;
                    }
                }
                \uIf{REALLOC\_FLAG = $false$}
                {
                    \Return{true}\;
                }
            }
        }
    }
}
\Return{false}\;
% \SetKwBlock{Begin}{function}{end function}
% \Begin($\text{detectRule2.5} {(} G {)}$)
% {
    
% }
\caption{Double-Free}
\label{algo:alg2.5}
\end{algorithm}

% \begin{algorithm}
% \caption{Double-Free}
% \label{algo:alg2.5}

% \begin{flushleft}
% %\vspace{1em}
% \textbf{PROPERTY KEYS}\\
% $dest$: Key denoting the destination buffer of an allocation function call\\
% \textbf{ACRONYMS}\\
% DF: De-allocation Function call\\
% PD: Post-Dominance\\
% \textbf{Begin}
% \begin{algorithmic}[1]
% \STATE Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = AF\}
% \FOR{node $x$ in $V'$}
%     \STATE Let $b$ $\gets$ $\mu(x, dest)$
%     \STATE Let $DA_{b} \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = DF and $\mu(v, arg\_dest)=b$\}
%     \FOR{$v$ in $DA_{b}$}
%         \FOR{$u$ in $DA_{b}$}
%             \IF{$(u, v) \in E$ and $\lambda((u, v)) = $ PD}
%                 \STATE REALLOC\_FLAG $\gets$ $false$
%                 \FOR{$w$ in $V'$}
%                     \IF{$\mu(w, dest) = b$ and $(u, w) \in E$ and $\lambda((u, w)) = $ PD and $(w, v) \in E$ and $\lambda((w, v)) = $ PD}
%                         \STATE REALLOC\_FLAG $\gets$ $true$
%                     \ENDIF
%                 \ENDFOR
%                 \IF{REALLOC\_FLAG = $false$}
%                     \STATE return $true$
%                 \ENDIF
%             \ENDIF
%         \ENDFOR
%     \ENDFOR
% \ENDFOR
% \STATE return $false$

% %\EndWhile
% \end{algorithmic}
% \textbf{End}
% \end{flushleft}
% \end{algorithm}
In Algorithm~\ref{algo:alg2.5}, Line 2 iterates through every node $x$ in $V'$ where $V'$ is the set of nodes representing an allocation function (AF) call (e.g., a call to \texttt{malloc}) (Line 1). Line 3 retrieves the destination buffer $b$ of the allocation function call. Line 4 retrieves the set of Nodes ($DA_{b}$) that deallocate buffer $b$. Lines 5-7 look for two nodes $u \in DA_{b}$  and $v \in DA_{b}$ where $v$ post-dominates $u$, meaning there is a deallocation of buffer $b$ in node $v$ after node $u$ previously also deallocates buffer $b$. However, the component still needs to ensure that buffer $b$ never gets reallocated between nodes $u$ and $v$ to say that the vulnerability is present. Lines 8-13 look for a node $w$ that represents an allocation function call for buffer $b$ and further checks if $w$ post-dominates $u$ and is post-dominated by $v$. If so then it means that node $w$ reallocates buffer $b$ between nodes $u$ and $v$. If no such node $w$ is found, then the component concludes that the sample contains the "Double-Free" vulnerability.

==> detection_algorithms/dealloc/use_after_free.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwIn{$G=( V,E, \lambda, \mu )$ representing the CPG constructed from the sample code}
\KwOut{Boolean value indicating whether the feature exists in the sample\\
\textbf{Begin}}
Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = AF\}\;
\For{node $x$ in $V'$}
{
    Let $b$ $\gets$ $\mu(x, dest)$\;
    Let $DA_{b} \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = DF and $\mu(v, arg\_dest)=b$\}\;
    Let node $y$ $\gets$ node $v \in V$ if $((x,v) \in E$ and $\lambda(x,v) = $ DEF and $\mu(v, symbol) = b$\;
    Let $USE_{b} \subset V$ $\gets$ \{$v$ for $v \in V$ if $(v, y) \in E$ and $\lambda(v, y) = $ USE\}\;
    \For{node $v$ in $USE_{b}$}
    {
        \For{node $u$ in $DA_{b}$}
        {
            \uIf{$(u, v) \in E$ and $\lambda(u, v) = $ PD}
            {
                REALLOC\_FLAG $\gets$ $false$\;
                \For{node $w$ in $V'$}
                {
                    \uIf{$\mu(w, dest) = b$ and $(u, w) \in E$ and $\lambda(u, w) = $ PD and $(w, v) \in E$ and $\lambda(w, v) = $ PD}
                    {
                        REALLOC\_FLAG $\gets$ $true$\;
                    }
                }
                \uIf{REALLOC\_FLAG = $false$}
                {
                    \Return{true}\;
                }
            }
        }
    }
}
\Return{false}\;
% \SetKwBlock{Begin}{function}{end function}
% \Begin($\text{detectRule2.6} {(} G {)}$)
% {
    
% }
\caption{Use-After-Free}
\label{algo:alg2.6}
\end{algorithm}

% \begin{algorithm}
% % \caption{Use-After-Free}
% % \label{algo:alg2.6}

% \begin{flushleft}
% %\vspace{1em}
% \textbf{PROPERTY KEYS}\\
% $symbol$: Key denoting the variable declared in a node\\
% \textbf{ACRONYMS}\\
% DEF: Definition of a variable\\
% USE: Use of a variable\\
% \textbf{Begin}
% \begin{algorithmic}[1]
% \STATE Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = AF\}
% \FOR{node $x$ in $V'$}
%     \STATE Let $b$ $\gets$ $\mu(x, dest)$
%     \STATE Let $DA_{b} \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = DF and $\mu(v, arg\_dest)=b$\}
%     \STATE Let node $y$ $\gets$ node $v \in V$ if $((x,v) \in E$ and $\lambda((x,v)) = $ DEF and $\mu(v, symbol) = b$
%     \STATE Let $USE_{b} \subset V$ $\gets$ \{$v$ for $v \in V$ if $(v, y) \in E$ and $\lambda((v, y)) = $ USE\}
%     \FOR{$v$ in $USE_{b}$}
%         \FOR{$u$ in $DA_{b}$}
%             \IF{$(u, v) \in E$ and $\lambda((u, v)) = $ PD}
%                 \STATE REALLOC\_FLAG $\gets$ $false$
%                 \FOR{$w$ in $V'$}
%                     \IF{$\mu(w, dest) = b$ and $(u, w) \in E$ and $\lambda((u, w)) = $ PD and $(w, v) \in E$ and $\lambda((w, v)) = $ PD}
%                         \STATE REALLOC\_FLAG $\gets$ $true$
%                     \ENDIF
%                 \ENDFOR
%                 \IF{REALLOC\_FLAG = $false$}
%                     \STATE return $true$
%                 \ENDIF
%             \ENDIF
%         \ENDFOR
%     \ENDFOR
% \ENDFOR
% \STATE return $false$

% %\EndWhile
% \end{algorithmic}
% \textbf{End}
% \end{flushleft}
% \end{algorithm}
In Algorithm~\ref{algo:alg2.6}, Line 2 iterates through every node $x$ in $V'$ where $V'$ is the set of nodes representing an allocation function (AF) call (e.g., a call to \texttt{malloc}) (Line 1). Line 3 retrieves the destination buffer $b$ of the allocation function call. Line 4 retrieves the set of Nodes ($DA_{b}$) that deallocate buffer $b$. Line 5 retrieves node $y$ representing the variable declaration statement for buffer $b$. Line 6 retrieves the set of CPG nodes ($USE_{b}$) that use buffer $b$. Lines 7-9 look for two nodes $u \in DA_{b}$ and $v\in USE_{b}$ where $v$ post-dominates $u$, meaning there is a use of buffer $b$ in node $v$ after node $u$ previously deallocates buffer $b$. Lines 10-15 look for a node $w$ that represents an allocation function call for buffer $b$ and further checks if $w$ post-dominates $u$ and is post-dominated by $v$. If so then it means that node $w$ reallocates buffer $b$ between nodes $u$ and $v$. If no such node $w$ is found, then the component concludes that the sample contains the "Use-After-Free" vulnerability.

==> detection_algorithms/keys_acros.tex <==
To facilitate our implementation of \textit{VIPer}, we extended the property function $\mu$'s capabilities to retrieve and set additional properties of nodes and edges. We list these additional property keys and values (as acronyms) used by property function $\mu$ in  Table~\ref{tab:cpg_keys}. The first half of the table lists the keys used by $\mu$ when retrieving properties, and the second half of the table lists the values returned by $\mu$. For example, to retrieve the value of the property ``type'' (see the first key in Table~\ref{tab:cpg_keys}) for node $v$, we will use the notation $\mu(v, type)$ and if the returned value is ``WF'' (see the first value in Table~\ref{tab:cpg_keys}), it means that node $v$ represents a buffer write function call.

\begin{table*}[htbp]
\centering
% \tiny
% \resizebox{\linewidth}{!}{%
\caption{Property keys and values (as acronyms) for the property function $\mu$}
\begin{tabular}{clll}
% {|p{0.15\linewidth}|p{0.15\linewidth}|p{0.60\linewidth}|}
\toprule
& \textbf{Property} & \textbf{Node/Edge} & \textbf{Meaning}\\
\midrule
\midrule
\multirow{16}{*}{\rotatebox[origin=c]{90}{Key}} & $type$ & Node & Denotes what the node represents \\
% \hline
& $arg\_dest$ & Node & Denotes the argument representing the destination buffer ($d$) in a buffer write function call \\
% \hline
& $arg\_src$ & Node & Denotes the argument representing the source buffer ($s$) in a buffer write function call \\
% \hline
& $arg\_count$ & Node & Denotes the argument representing the number of bytes ($n$) to write in a buffer write function call \\
% \hline
& $len$ & Node & Denotes the length assigned to a buffer in a node \\ 
% \hline
& $dest$ & Node & Denotes the destination buffer of an allocation function call \\ 
% \hline
& $dest\_arr$ & Node & Denotes the destination array for a node representing an array indexing operation \\
% \hline
& $dest\_index$ & Node & Denotes the index used to access the destination array in a node representing an array indexing operation \\
% \hline
& $src\_arr$ & Node & Denotes the source array for a node representing an array indexing operation \\
% \hline
& $src\_index$ & Node & Denotes the index used to access the source array in a node representing an array indexing operation \\
% \hline
& $symbol$ & Node & Denotes the variable declared in a node \\
% \hline
& $operator$ & Node & Denotes the operator used in a node representing a Relational Expression \\
% \hline
& $identifier$ & Node & Denotes the variable used in a node representing a Relational Expression \\
% \hline
& $literal$ & Node & Denotes the literal value used in a node representing a Relational Expression \\
% \hline
& $loc$ & Node & Denotes the source code line where the CPG node \\
% \hline
& $var$ &Edge & Denotes the variable associated with a data dependence edge \\
\midrule
\midrule
\multirow{15}{*}{\rotatebox[origin=c]{90}{Value}} & $WF$ & Node & Buffer write function call. Corresponds to what a node represents.\\
& $CF$ & Node & Buffer copy function call. Corresponds to what a node represents.\\
& $AF$ & Node & Allocation Function call. Corresponds to what a node represents.\\
& $DF$ & Node & De-allocation Function call. Corresponds to what a node represents.\\
& $SF$ & Node & Sensitive API or function call. Corresponds to what a node represents.\\
& $AD$ & Node & Array Declaration. Corresponds to what a node represents.\\
& $AI$ & Node & Array Indexing operation. Corresponds to what a node represents.\\
& $RE$ & Node & Relational Expression. Corresponds to what a node represents.\\
& $GE$ & Node & Greater than or Equals relation. Corresponds to the comparison used in a node representing a Relational Expression.\\
& $GT$ & Node & Is greater than relation. Corresponds to the comparison used in a node representing a Relational Expression.\\
& $DD$ & Edge & Edge denoting Data Dependence.\\
& $CD$ & Edge & Edge denoting Control Dependence.\\
& $PD$ & Edge & Edge denoting Post-Dominance.\\
& $DEF$ & Edge & Edge denoting Definition of a variable.\\
& $USE$ & Edge & Edge denoting Use of a variable.\\
\bottomrule
\end{tabular}
\label{tab:cpg_keys}
        
\end{table*}
% All the acronyms we used to describe property values of nodes and edges are described below:

% \textbf{ACRONYMS}\\



==> detection_algorithms/num_range/underread.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwIn{$G=( V,E, \lambda, \mu )$ representing the CPG constructed from the sample code}
\KwOut{Boolean value indicating whether the feature exists in the sample\\
\textbf{Begin}}
Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = AI\}\;
\For{node $v$ in $V'$}
{
    Let $b$ $\gets$ $\mu(v, src\_arr)$\;
    Let $idx$ $\gets$ $\mu(v, src\_index)$\;
    Let $IN_{v}^{CD} \subset V$ $\gets$ \{$u$ for $u \in V$ if $(u, v) \in E$ and $\lambda(u, v) = $ CD\}\;
    \For{$u$ in $IN_{v}^{CD}$}
    {
        \uIf{$\mu(u, type) =$ RE and $((\mu(u, operator)=$ GE and $\mu(u, identifier) = idx$ and $\mu(u, literal) = 0)$ or $(\mu(u, operator)=$ GT and $\mu(u, identifier) = idx$ and $\mu(u, literal) = -1))$}
        {
            \Return{false}\;
        }
    }
}
\Return{true}\;
% \SetKwBlock{Begin}{function}{end function}
% \Begin($\text{detectRule2.8} {(} G {)}$)
% {
    
% }
\caption{Buffer Under-read}
\label{algo:alg2.8}
\end{algorithm}

% \begin{algorithm}
% \caption{Buffer Under-read}
% \label{algo:alg2.8}

% \begin{flushleft}
% %\vspace{1em}
% \textbf{PROPERTY KEYS}\\
% $src\_arr$: Key denoting the source array for a node representing an array indexing operation\\
% $src\_index$: Key denoting the index used to access the source array in a node representing an array indexing operation\\
% \textbf{Begin}
% \begin{algorithmic}[1]
% \STATE Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = AI\}
% \FOR{node $v$ in $V'$}
%     \STATE Let $b$ $\gets$ $\mu(v, src\_arr)$
%     \STATE Let $idx$ $\gets$ $\mu(v, src\_index)$
%     \STATE Let $icdn \subset V$ $\gets$ \{$u$ for $u \in V$ if $(u, v) \in E$ and $\lambda((u, v)) = $ CD\}
%     \FOR{$u$ in $icdn$}
%         \IF{$\mu(u, type) =$ RE and $((\mu(u, operator)=$ GE and $\mu(u, identifier) = idx$ and $\mu(u, literal) = 0)$ or $(\mu(u, operator)=$ GT and $\mu(u, identifier) = idx$ and $\mu(u, literal) = -1))$}
%         \STATE return $false$
%         \ENDIF
%     \ENDFOR
% \ENDFOR
% \STATE return $true$

% %\EndWhile
% \end{algorithmic}
% \textbf{End}
% \end{flushleft}
% \end{algorithm}
In Algorithm~\ref{algo:alg2.8}, Line 2 iterates through every node $v$ in $V'$ where $V'$ is the set of nodes representing an array indexing (AI) operation allocation (Line 1). Lines 3 and 4 retrieve the source array $b$ and the index ($idx$) used to access $b$ in the array indexing operation, respectively. Line 5 in the algorithm retrieves the start nodes of all the incoming control dependence (CD) edges of node $v$ (i.e., $IN_{v}^{CD}$). Lines 6-8 iterate through the retrieved control dependence edges and check if an edge's start node $u$ contains a "greater than or equals" (GE) comparison between $idx$ and $0$ or an "is greater than" (GT) comparison between $idx$ and $-1$. If no such comparisons are found, the component concludes that the sample contains the "Buffer Under-read" vulnerability.

==> detection_algorithms/num_range/underwrite.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwIn{$G=( V,E, \lambda, \mu )$ representing the CPG constructed from the sample code}
\KwOut{Boolean value indicating whether the feature exists in the sample\\
\textbf{Begin}}
Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = AI\}\;
\For{node $v$ in $V'$}
{
    Let $b$ $\gets$ $\mu(v, dest\_arr)$\;
    Let $idx$ $\gets$ $\mu(v, dest\_index)$\;
    Let $IN_{v}^{CD} \subset V$ $\gets$ \{$u$ for $u \in V$ if $(u, v) \in E$ and $\lambda(u, v) = $ CD\}\;
    \For{$u$ in $IN_{v}^{CD}$}
    {
        \uIf{$\mu(u, type) =$ RE and $((\mu(u, operator)=$ GE and $\mu(u, identifier) = idx$ and $\mu(u, literal) = 0)$ or $(\mu(u, operator)=$ GT and $\mu(u, identifier) = idx$ and $\mu(u, literal) = -1))$}
        {
            \Return{false}\;
        }
    }
}
\Return{true}\;
% \SetKwBlock{Begin}{function}{end function}
% \Begin($\text{detectRule2.7} {(} G {)}$)
% {
    
% }
\caption{Buffer Underwrite}
\label{algo:alg2.7}
\end{algorithm}

% \begin{algorithm}
% \caption{Buffer Underwrite}
% \label{algo:alg2.7}

% \begin{flushleft}
% %\vspace{1em}
% \textbf{PROPERTY KEYS}\\
% $dest\_arr$: Key denoting the destination array for a node representing an array indexing operation\\
% $dest\_index$: Key denoting the index used to access the destination array in a node representing an array indexing operation\\
% $operator$: Key denoting the operator used in a node representing a Relational Expression\\
% $identifier$: Key denoting the variable used in a node representing a Relational Expression\\
% $literal$: Key denoting the literal value used in a node representing a Relational Expression\\
% \textbf{ACRONYMS}\\
% AI: Array Indexing operation\\
% CD: Control Dependence\\
% RE: Relational Expression\\
% GE: Greater than or Equals\\
% GT: Is greater than\\
% \textbf{Begin}
% \begin{algorithmic}[1]
% \STATE Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = AI\}
% \FOR{node $v$ in $V'$}
%     \STATE Let $b$ $\gets$ $\mu(v, dest\_arr)$
%     \STATE Let $idx$ $\gets$ $\mu(v, dest\_index)$
%     \STATE Let $icdn \subset V$ $\gets$ \{$u$ for $u \in V$ if $(u, v) \in E$ and $\lambda((u, v)) = $ CD\}
%     \FOR{$u$ in $icdn$}
%         \IF{$\mu(u, type) =$ RE and $((\mu(u, operator)=$ GE and $\mu(u, identifier) = idx$ and $\mu(u, literal) = 0)$ or $(\mu(u, operator)=$ GT and $\mu(u, identifier) = idx$ and $\mu(u, literal) = -1))$}
%         \STATE return $false$
%         \ENDIF
%     \ENDFOR
% \ENDFOR
% \STATE return $true$

% %\EndWhile
% \end{algorithmic}
% \textbf{End}
% \end{flushleft}
% \end{algorithm}
In Algorithm~\ref{algo:alg2.7}, Line 2 iterates through every node $v$ in $V'$ where $V'$ is the set of nodes representing an array indexing (AI) operation allocation (Line 1). Lines 3 and 4 retrieve the destination array $b$ and the index ($idx$) used to access $b$ in the array indexing operation, respectively. Line 5 in the algorithm retrieves the start nodes of all the incoming control dependence (CD) edges of node $v$ (i.e, $IN_{v}^{CD}$). Lines 6-8 iterate through the retrieved control dependence edges and check if an edge's start node $u$ contains a "greater than or equals" (GE) comparison between $idx$ and $0$ or an "is greater than" (GT) comparison between $idx$ and $-1$. If no such comparisons are found, the component concludes that the sample contains the "Buffer Underwrite" vulnerability.

==> detection_algorithms/overflow/off-by-one.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwIn{$G=( V,E, \lambda, \mu )$ representing the CPG constructed from the sample code}
\KwOut{Boolean value indicating whether the feature exists in the sample\\
\textbf{Begin}}
Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = WF\}\;
\For{node $v$ in $V'$}
{
    Let $d$ $\gets$ $\mu(v, arg\_dest)$\;
    Let $n$ $\gets$ $\mu(v, arg\_count)$\;
    Let $IN_{v}^{DD} \subset V$ $\gets$ \{$u$ for $u \in V$ if $(u, v) \in E$ and $\lambda(u, v) = $ DD and $\mu((u,v), var) = d$ \}\;
    \For{$u$ in $IN_{v}^{DD}$}
    {
        \uIf{$\mu(u, type)$ = AF or $\mu(u, type)$ = AD}
        {
            Let $LEN_{d}$ $\gets$ $\mu(u, len)$\;
            \uIf{$n = LEN_{d} + 1$}
            {
                \Return{true}\;
            }
        }
    }
}
\Return{false}\;
% \SetKwBlock{Begin}{function}{end function}
% \Begin($\text{detectRule2.3} {(} G {)}$)
% {
    
% }
\caption{Off-by-one Error}
\label{algo:alg2.3}
\end{algorithm}

% \begin{algorithm}
% % \caption{Off-by-one Error}
% % \label{algo:alg2.3}

% \begin{flushleft}
% %\vspace{1em}
% \textbf{Begin}
% \begin{algorithmic}[1]
% \STATE Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = WF\}
% \FOR{node $v$ in $V'$}
%     \STATE Let $d$ $\gets$ $\mu(v, arg\_dest)$
%     \STATE Let $n$ $\gets$ $\mu(v, arg\_count)$
%     \STATE Let $iddn \subset V$ $\gets$ \{$u$ for $u \in V$ if $(u, v) \in E$ and $\lambda((u, v)) = $ DD and $\mu((u,v), var) = d$ \}
%     \FOR{$u$ in $iddn$}
%         \IF{$\mu(u, type)$ = AF or $\mu(u, type)$ = AD}
%             \STATE Let $LEN_{d}$ $\gets$ $\mu(u, len)$
%             \IF{$n = LEN_{d} + 1$}
%                 \STATE return $true$
%             \ENDIF
%         \ENDIF
%     \ENDFOR
% \ENDFOR
% \STATE return $false$

% %\EndWhile
% \end{algorithmic}
% \textbf{End}
% \end{flushleft}
% \end{algorithm}
In Algorithm~\ref{algo:alg2.3}, Line 2 iterates through every node $v$ in $V'$ where $V'$ is the set of nodes representing a buffer write function (WF) call (e.g., a call to \texttt{memcpy}) (Line 1). Lines 3 and 4 in the algorithm retrieve the destination buffer ($d$) and the number of bytes to write ($n$) in the function call, respectively. Line 5 in the algorithm retrieves the start nodes of all the incoming data dependence (DD) edges of node $v$ with respect to the destination buffer $d$ (i.e., $IN_{v}^{DD}$). Lines 6-10 iterate through the retrieved data dependence edges and check if an edge's start node $u$ represents an allocation function (AF) or an array declaration (AD). If so, it further checks whether the number of bytes to write ($n$) according to node $v$ exceeds the length defined at node $u$ by exactly one (Line 9). If true, it concludes that the sample contains the vulnerability “Off-by-one Error”.

==> detection_algorithms/overflow/over_read.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwIn{$G=( V,E, \lambda, \mu )$ representing the CPG constructed from the sample code}
\KwOut{Boolean value indicating whether the feature exists in the sample\\
\textbf{Begin}}
Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = CF\}\;
\For{node $v$ in $V'$}
{
    Let $s$ $\gets$ $\mu(v, arg\_src)$\;
    Let $n$ $\gets$ $\mu(v, arg\_count)$\;
    Let $IN_{v}^{DD} \subset V$ $\gets$ \{$u$ for $u \in V$ if $(u, v) \in E$ and $\lambda(u, v) = $ DD and $\mu((u,v), var) = s$ \}\;
    \For{$u$ in $IN_{v}^{DD}$}
    {
        \uIf{$\mu(u, type)$ = AF or $\mu(u, type)$ = AD}
        {
            Let Let $LEN_{s}$ $\gets$ $\mu(u, len)$\;
            \uIf{$n > LEN_{s}$}
            {
                \Return{true}\;
            }
        }
    }
}
\Return{false}\;
% \SetKwBlock{Begin}{function}{end function}
% \Begin($\text{detectRule2.4} {(} G {)}$)
% {
    
% }
\caption{Buffer Over-read}
\label{algo:alg2.4}
\end{algorithm}

% \begin{algorithm}
% \caption{Buffer Over-read}
% \label{algo:alg2.4}

% \begin{flushleft}
% %\vspace{1em}
% \textbf{ACRONYMS}\\
% CF: Buffer copy function call\\
% \textbf{Begin}
% \begin{algorithmic}[1]
% \STATE Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = CF\}
% \FOR{node $v$ in $V'$}
%     \STATE Let $s$ $\gets$ $\mu(v, arg\_src)$
%     \STATE Let $n$ $\gets$ $\mu(v, arg\_count)$
%     \STATE Let $iddn \subset V$ $\gets$ \{$u$ for $u \in V$ if $(u, v) \in E$ and $\lambda((u, v)) = $ DD and $\mu((u,v), var) = s$ \}
%     \FOR{$u$ in $iddn$}
%         \IF{$\mu(u, type)$ = AF or $\mu(u, type)$ = AD}
%             \STATE Let $LEN_{s}$ $\gets$ $\mu(u, len)$
%             \IF{$n > LEN_{s}$}
%                 \STATE return $true$
%             \ENDIF
%         \ENDIF
%     \ENDFOR
% \ENDFOR
% \STATE return $false$

% %\EndWhile
% \end{algorithmic}
% \textbf{End}
% \end{flushleft}
% \end{algorithm}
In Algorithm~\ref{algo:alg2.4}, Line 2 iterates through every node $v$ in $V'$ where $V'$ is the set of nodes representing a buffer copy function (CF) call (e.g., a call to \texttt{strncpy}) (Line 1). Lines 3 and 4 in the algorithm retrieve the source buffer ($s$) and the number of bytes to read ($n$) in the function call, respectively. Line 5 in the algorithm retrieves the start nodes of all the incoming data dependence (DD) edges of node $v$ with respect to the source buffer $s$ (i.e., $IN_{v}^{DD}$). Lines 6-10 iterate through the retrieved data dependence edges and check if an edge's start node $u$ represents an allocation function (AF) or an array declaration (AD). If so, it further checks whether the number of bytes to read ($n$) according to node $v$ exceeds the length defined at node $u$ (Line 9). If true, it concludes that the sample contains the vulnerability “Buffer Over-read”.

==> detection_algorithms/overflow/src_size.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwIn{$G=( V,E, \lambda, \mu )$ representing the CPG constructed from the sample code}
\KwOut{Boolean value indicating whether the feature exists in the sample\\
\textbf{Begin}}
Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = WF\}\;
\For{node $v$ in $V'$}
{
    Let $d$ $\gets$ $\mu(v, arg\_dest)$\;
    Let $s$ $\gets$ $\mu(v, arg\_src)$\;
    Let $n$ $\gets$ $\mu(v, arg\_count)$\;
    Let $IN_{v}^{DD,s} \subset V$ $\gets$ \{$u$ for $u \in V$ if $(u, v) \in E$ and $\lambda(u, v) = $ DD and $\mu((u,v), var) = s$ \}\;
    $LEN_{s}$ $\gets$ \{\}\;
    \For{$u$ in $IN_{v}^{DD,s}$}
    {
        \uIf{$\mu(u, type)$ = AF or $\mu(u, type)$ = AD}
        {
            Let $len_{s}$ $\gets$ $\mu(u, len)$\;
            $LEN_{s}$ $\gets$ $LEN_{s} \cup$ \{$len_{s}$\}\;
        }
    }
    Let $IN_{v}^{DD,d} \subset V$ $\gets$ \{$u$ for $u \in V$ if $(u, v) \in E$ and $\lambda(u, v) = $ DD and $\mu((u,v), var) = d$ \}\;
    \For{$u$ in $IN_{v}^{DD,d}$}
    {
        \uIf{$\mu(u, type)$ = AF or $\mu(u, type)$ = AD}
        {
            Let $LEN_{d}$ $\gets$ $\mu(u, len)$\;
            \uIf{$(n > LEN_{d})$ and $(n \in LEN_{s})$}
            {
                \Return{true}\;
            }
        }
    }
}
\Return{false}\;
% \SetKwBlock{Begin}{function}{end function}
% \Begin($\text{detectRule2.2} {(} G {)}$)
% {
    
% }
\caption{Buffer Access Using Size of Source Buffer}
\label{algo:alg2.2}
\end{algorithm}

% \begin{algorithm}
% \caption{Buffer Access Using Size of Source Buffer}
% \label{algo:alg2.2}

% \begin{flushleft}
% %\vspace{1em}
% \textbf{PROPERTY KEYS}\\
% $arg\_src$: Key denoting the argument representing the source buffer ($s$) in a buffer write function call\\
% \textbf{Begin}
% \begin{algorithmic}[1]
% \STATE Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = WF\}
% \FOR{node $v$ in $V'$}
%     \STATE Let $d$ $\gets$ $\mu(v, arg\_dest)$
%     \STATE Let $s$ $\gets$ $\mu(v, arg\_src)$
%     \STATE Let $n$ $\gets$ $\mu(v, arg\_count)$
%     \STATE Let $iddns \subset V$ $\gets$ \{$u$ for $u \in V$ if $(u, v) \in E$ and $\lambda((u, v)) = $ DD and $\mu((u,v), var) = s$ \}
%     \STATE $LEN_{s}$ $\gets$ \{\}
%     \FOR{$u$ in $iddns$}
%         \IF{$\mu(u, type)$ = AF or $\mu(u, type)$ = AD}
%             \STATE Let $len_{s}$ $\gets$ $\mu(u, len)$
%             \STATE $LEN_{s}$ $\gets$ $LEN_{s} \cup$ \{$len_{s}$\}
%         \ENDIF
%     \ENDFOR
%     \STATE Let $iddnd \subset V$ $\gets$ \{$u$ for $u \in V$ if $(u, v) \in E$ and $\lambda((u, v)) = $ DD and $\mu((u,v), var) = d$ \}
%     \FOR{$u$ in $iddnd$}
%         \IF{$\mu(u, type)$ = AF or $\mu(u, type)$ = AD}
%             \STATE Let $LEN_{d}$ $\gets$ $\mu(u, len)$
%             \IF{$(n > LEN_{d})$ and $(n \in LEN_{s})$}
%                 \STATE return $true$
%             \ENDIF
%         \ENDIF
%     \ENDFOR
% \ENDFOR
% \STATE return $false$

% %\EndWhile
% \end{algorithmic}
% \textbf{End}
% \end{flushleft}
% \end{algorithm}
In Algorithm~\ref{algo:alg2.2}, Line 2 iterates through every node $v$ in $V'$ where $V'$ is the set of nodes representing a buffer write function (WF) call (e.g., a call to \texttt{memcpy}) (Line 1). Lines 3-5 in the algorithm retrieve the destination buffer ($d$), the source buffer ($s$), and the number of bytes to write ($n$) in the function call, respectively. Line 6 retrieves the start nodes of all the incoming data dependence (DD) edges of node $v$ with respect to the source buffer $s$ (i.e., $IN_{v}^{DD,s}$). Lines 7-11 iterate through the edges retrieved in Line 6 and check if an edge's start node $u$ represents an allocation function (AF) or an array declaration (AD). If so, it extracts the length defined in node $u$ as a length for the source buffer $s$. Similar to line 6, line 12 retrieves the start nodes of all the incoming DD edges of node $v$ with respect to the destination buffer $d$ (i.e., $IN_{v}^{DD,d}$). Lastly, 13-17 iterate through the edges retrieved in line 12 and check if an edge's start node $u$ represents an allocation function (AF) or an array declaration (AD). If so, it further checks whether the number of bytes to write ($n$) according to node $v$ exceeds the length defined at node $u$ and equals a defined length for the source buffer (Line 16). If true, it concludes that the sample contains the vulnerability “Buffer Access Using Size of Source Buffer”.

==> detection_algorithms/sensi_read_write/sensi_r_w.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwIn{
\\$G=( V,E, \lambda, \mu )$ representing the CPG constructed from the sample code
\\$Y$ representing the line level ground truth of the sample where the vulnerable line numbers are provided.}
\KwOut{Boolean value indicating whether the feature exists in the sample\\
\textbf{Begin}}
Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = SF\}\;
\For{node $v$ in $V'$}
{
    Let $\mathcal{L}$ $\gets$ $\mu(v, loc)$\;
    \uIf{$\mathcal{L} \in Y$}
    {
        \Return{true}\;
    }
}
\Return{false}\;
% \SetKwBlock{Begin}{function}{end function}
% \Begin($\text{detectRule2.9} {(} G {)}$)
% {
    
% }
\caption{Sensitive Read/Write Vulnerability}
\label{algo:alg2.9}
\end{algorithm}

% \begin{algorithm}
% \caption{Sensitive Read/Write Vulnerability}
% \label{algo:alg2.9}

% \begin{flushleft}
% %\vspace{1em}
% \textbf{Input}\\
% $G=( V,E, \lambda, \mu )$ representing the CPG constructed from the sample code\\
% $Y$ representing the line level ground truth of the sample where the vulnerable line numbers are provided.\\
% \textbf{PROPERTY KEYS}\\
% $loc$: Key denoting the source code line where the CPG node \\
% \textbf{ACRONYMS}\\
% SF: Sensitive API or function call\\
% \textbf{Begin}
% \begin{algorithmic}[1]
% \STATE Let $V' \subset V$ $\gets$ \{$v$ for $v \in V$ if $\mu(v, type)$ = SF\}
% \FOR{node $v$ in $V'$}
%     \STATE Let $\mathcal{L}$ $\gets$ $\mu(v, loc)$
%     \IF{$\mathcal{L} \in Y$}
%         \STATE return $true$
%     \ENDIF
% \ENDFOR
% \STATE return $false$

% %\EndWhile
% \end{algorithmic}
% \textbf{End}
% \end{flushleft}
% \end{algorithm}
In Algorithm~\ref{algo:alg2.9}, Line 2 iterates through every node $v$ in $V'$ where $V'$ is the set of nodes representing a sensitive API or function (SF) call (Line 1). Line 3 retrieves the location $\mathcal{L}$ of node $v$. Lines 4 and 5 check if the location is a vulnerable line. If so, the component concludes that the sample contains the "Sensitive Read/Write Vulnerability" vulnerability.

==> dummy_sections/definitions.tex <==
\section{Definitions}
\label{sec:definitions}
{
Definitions here.
}

==> dummy_sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
{
Introduction here.
}

==> prev/approach.tex <==
\section{Approach}
\label{sec:approach}
{
We design software source code transformations that target vulnerability features and model-specific weaknesses to evaluate whether the subject matters (i.e., VDT) are learning the vulnerability features we proposed and how susceptible they are to their model-specific weakness. This section will describe how we generate the transformations targeting a feature or a weakness.\\
\subsection{Feature Targeted Transformations}
\label{subsec:feat-trf}
{
Transformations that fall under this category target the vulnerability features described in Section \ref{sec:definitions}. To generate the transformations, we use the Code Property Graph~\cite{yamaguchi2014modeling} to detect the existence of a vulnerability feature in a function. Once we extract the samples in the database containing the vulnerability feature $\displaystyle X$, we apply transformations that enforce, remove, or preserve the detected feature(s). Detailed generation steps for each vulnerability feature are given below:\\
\textbf{Equality of Definition-Use:} We use the data dependence graph to determine the existence of a sample's "Equality of Definition-Use" property. The procedure goes as follows:\\
\begin{enumerate}
    \item We first determine the location of the following sensitive API calls: \texttt{\texttt{memcpy}, \texttt{strncpy}, \texttt{strcpy}, \texttt{wcsncpy}, \texttt{memset} and \texttt{wmemset}}.
    \item Next, we determine the definition used in the function call and traverse the function call's incoming data dependence edges to find the same definition's existence. If the definition is found, we check the label of the function. Since the Equality of Definition-Use property often fixes the vulnerability, we only consider the samples labeled as non-vulnerable. 
    \item Lastly, for each recorded sample, we apply three transformations. We change the definition to become unequal to (smaller than) the function call's use. Such a transformation should change the VDT's prediction to vulnerable. Next, we change the located definition and the function call's use, but we ensure they are equal. For a change like this, the VDT's prediction should remain non-vulnerable~\tuan{At the beginning of this subsection, it would be better if you categorize the transformations into prediction-preserving and prediction-inverting changes. Also, at each transformation type, you should mention what is the starting point for transforming i.e., from vul or non-vul example?}. For the last transformation, if the definition and the use contain numeric literals, we apply a mathematical operation transformation on the function call's use to reach mathematical equality to the definition. However, although mathematical equality can fix the vulnerability, we don't consider this a vulnerability feature since DL-based models do not learn them\cite{lu-etal-2023-survey, wallace-etal-2019-nlp}. Therefore, for the last type of transformation, the VDT should change its prediction to vulnerable. ~\tuan{the conclusion seems contradicting the previous sentence "we don't consider this a vulnerability feature"}
\end{enumerate}
\textbf{Inequality of Allocation-Deallocation:} We again use the data dependence graph of the function to determine whether the sample function has this property. To illustrate,  we'll break down the process into the steps below:
\begin{enumerate}
    \item First, we locate the call site for allocate functions \texttt{malloc}, \texttt{calloc}, and \texttt{alloca}. We record the call sites as allocation definitions for variable $\displaystyle X$.
    \item Next, we traverse the outgoing data dependency edges to look for a call to the function \texttt{free}.
    \item Once we locate the \texttt{free} function, we look further down the data dependency graph to locate a use of variable $\displaystyle X$. If the process locates a use further down the data dependence graph, we inspect the label of the function. Since we observe that the inequality of allocation-deallocation fixes the use after free vulnerability, we only consider the samples labeled as vulnerable.
    \item After determining the existence of the property, we again apply three transformations to the sample. First, we replace the call to \texttt{free} with \texttt{free(NULL)}. This is a safe operation and eliminates the use-after-free vulnerability. For such transformations, the VDT should change its prediction to non-vulnerable. Next, we change the line where we locate the use of the variable $\displaystyle X$ after it's been freed and replace the use line with a \texttt{printf} call with an empty string. This transformation is also safe and eliminates the vulnerability; thus, the VDT should change its prediction to non-vulnerable. The third transformation involves changing the function call to \texttt{malloc}, \texttt{calloc}, or \texttt{alloca} and assigning \texttt{NULL} to variable $\displaystyle X$. This transformation doesn't resolve the vulnerability, so in this case, the VDT should still predict the sample as vulnerable.  
\end{enumerate}
\textbf{Relevant Literal Values:} We identified several relevant literals for the task of vulnerability detection. For buffer underwrite vulnerabilities, we identify the literals $\displaystyle 0$ and $\displaystyle -1$ as relevant since they are often used in checking the lower bound of array access. We also observed that the fixes for improper access control/authorization vulnerabilities often involve comparisons with $\displaystyle NULL$ and truth value literal $\displaystyle 1$. To evaluate the VDT's comprehension of the feature, we generate the transformations in the following way:\\
\begin{enumerate}
    \item We first identify the vulnerable samples tagged as a buffer underwrite vulnerability and extract the index variable, $\displaystyle i$, used in the vulnerable line of code where the out-of-bounds array access occurs.
    \item Next, we traverse the incoming control dependence edges of the line to look for the conditions used to compare $\displaystyle i$ and the relevant literals $\displaystyle 0$ or $\displaystyle -1$. If a comparison doesn't exist, we select the samples for applying transformations and move on to the next step.
    \item Once we have selected the samples, we apply four transformations to evaluate the VDT's comprehension of relevant literal values. First, we add a "Greater than or Equal to" comparison between $\displaystyle i$ and $\displaystyle 0$. Such a transformation should fix the vulnerability; therefore, the VDT should change its prediction to "non-vulnerable." Second, we add a "Greater than" comparison between $\displaystyle i$ and $\displaystyle -1$. For the same reason as the previous transformation, the VDT should change its prediction to "non-vulnerable." Third, we extract the size, $\displaystyle l$, for the array that's causing the buffer-underwrite vulnerability and randomly choose a negative value $\displaystyle cmp\_val= 2\times l\times ( -1)$ and add a "Greater than" comparison between $\displaystyle i$ and $\displaystyle cmp\_val$~\tuan{does the transformation of complex math operators seem reasonable regarding that you cited some papers saying DL model cannot learn math operations?}. Such a transformation doesn't fix the vulnerability or introduce the "Equality of Definition-Use" property in the sample. Therefore, the VDT should keep its prediction as "vulnerable." For the fourth transformation, we add a "Greater than or Equal to" comparison between $\displaystyle i$ and $\displaystyle ( cmp\_val-cmp\_val)$. Although $\displaystyle ( cmp\_val-cmp\_val)$ evaluates to $\displaystyle 0$ and this transformation fixes the vulnerability, the VDT should retain the prediction of "vulnerable" since we consider all mathematical operations irrelevant for DL-based learning.
\end{enumerate}
\textbf{Sensitive APIs:} To evaluate the comprehension of sensitive APIs, we perform the following steps:\\
\begin{enumerate}
    \item First, we select all the vulnerable samples that contain at least one vulnerable line of code involving a function call to one of our listed sensitive APIs. We also inspect other vulnerable lines in the sample to check if they perform an array access operation. If such lines don't exist, we can confidently contribute the vulnerability to the function call and select the sample for transformation.
    \item Next, we replace the function call to the sensitive API on the selected samples with a dummy harmless function. Since, in the previous step, we attribute the vulnerability to the sensitive API, the VDT should change its prediction to "non-vulnerable."
\end{enumerate}
% \textbf{Condition Comprehensiveness:}\\
}

\subsection{Weakness Targeted Transformations}
\label{subsec:weakness-trf}
{
We also evaluate the susceptibility of the VDTs to their model-specific weakness. Therefore, we generate transformations for the weaknesses as well. However, we can assess several weaknesses by measuring the comprehension of certain vulnerability features. We present the process to generate the transformations targeting the weaknesses of token-based and graph-based approaches.\\
\textbf{Token-Based Approaches:} We identify and generate transformations for the following weaknesses of token-based approaches:\\
\begin{itemize}
    \item \textbf{Token Relevance:} To evaluate whether token-based approaches are learning irrelevant tokens from the source code, we do a simple transformation of adding and removing indentation from all samples in the test dataset. Ideally, a token-based VDT should retain its reported accuracy score even after the transformation since these transformations don't impact the sample's label.
    \item \textbf{Project-Specific Vocabulary:} While learning project-specific vocabulary can help make vulnerability predictions for the projects involved in training, it does not help detect vulnerabilities in unseen data from different projects. Therefore, we perform a symbolization of the software source code using the methodology proposed by Zhen Li~\cite{li2018vuldeepecker}. Like the transformations above, the VDT should retain the accuracy measures since symbolization has nothing to do with vulnerabilities and only introduces a project-context-free vocabulary.~\tuan{this weakness may also happen in graph-based approaches as they encode the token name in the graph's nodes?}.
\end{itemize}
\textbf{Graph-Based Approaches:} To assess the susceptibility of Graph-based approaches, we identify and generate transformations for the following weaknesses:\\
\begin{itemize}
    \item Following the description provided in Section \ref{sec:definitions}, we evaluate whether the graph-based VDT is learning only the existence of edges from its comprehension of the "Equality of Definition-Use" and "Inequality of Allocation-Deallocation" properties. If the accuracy of the VDT doesn't drop for at least one of those two properties, we will conclude that the VDT is learning more than just the existence of edges.
    \item Since SVD datasets do not contain information about runtime program states, we choose a program state (condition satisfiability) and generate transformations to assess its impact on the prediction. We first locate vulnerable \texttt{if} statement conditions for buffer-underwrite vulnerabilities using the same method we used to extract the condition nodes while evaluating the comprehension of relevant literal values. Next, we transform the \texttt{if} statement to contain an unsatisfiable condition (i.e., \texttt{5!=5}). Due to the unsatisfiability of the condition, the vulnerable line of code will not be executed during runtime. However, the VDT should still predict the sample as vulnerable since information about condition satisfiability is unavailable from SVD datasets~\tuan{this weakness may also happen in token-based approaches?}.
\end{itemize}
}

}

==> prev/definitions.tex <==
\section{Definitions}
\label{sec:definitions}
{\saad{Here, I wouldn't say ``we observed that...'', instead we can say: There are certain properties in the code that directly/strongly correlated towards a target label and also represent the cause of vulnerability. We call these properties as vulnerability features...}
We observed that in SVD datasets, source code samples often have properties detectable with static analysis that directly contribute to the sample's label (i.e., whether the sample is vulnerable or not).\saad{here, we need to mention that we are talking about SVDT models that are learning wrong properties which, when refactored, lead to change in their outcomes} In all cases where they are directly responsible for causing/fixing the vulnerabilities, only violating or enforcing the feature is sufficient to change the sample's label. We term these features as Vulnerability Features. Similarly, we also observed features (again detectable with static analysis) in samples that correlate with the sample's label but do not explain why the sample is vulnerable/non-vulnerable. We follow the terminology used by Rahman, Md Mahbubur, et al.\cite{rahman2023towards} and call them Spurious Features. We understand that\saad{we believe that...} based on the underlying approach (Graph-based or Token-based), the VDT may suffer from inadequate preprocessing of the samples, leading them to learn these spurious features and make predictions based on them.\\
For this study, we detected four Vulnerability Features using static analysis: Equality of Definition-Use, Equality of Allocation-Deallocation, Condition-checking Literals\saad{is it boundary or condition-checking?}, and Sensitive APIs. We formalized the Spurious Features according to the underlying strategy (Graph-based or Token-based). For Token-based approaches, we detected the spurious features: Token Relevance and Project-Specific Vocabulary. For Graph-based approaches, we detected Edge Existence and Path Coverage Information. We will define each Vulnerability Feature and Spurious Feature for the rest of the section. \saad{need to explain what table 1 is about.}
\begin{table*}[t]
\caption{Vulnerability Features}
\label{tab:vul_feat}
\centering
\begin{tabular}{|m{4.5cm}|m{3.5cm}|m{3.5cm}|m{4cm}|}
\hline
\textbf{Vulnerability Feature} & \textbf{Relevance on Vulnerable Samples} & \textbf{Relevance on Non-Vulnerable Samples} & \textbf{Impact upon Feature Removal} \\
\hline
Equality of Definition-Use & Low & High & The label should change from Non-Vulnerable to Vulnerable \\
\hline
Equality of Allocation-Deallocation before Use & High-Root Cause & None & The label should change from Vulnerable to Non-Vulnerable if the only root cause \\
\hline
Condition Checking Literals & Low & High & The label should change from Non-Vulnerable to Vulnerable \\
\hline
Sensitive APIs & Potentially High and should be determined through static analysis & None & If the impact is determined to be high, then the label should change Vulnerable to Non-Vulnerable \\
\hline

\end{tabular}
\end{table*}



\subsection{Vulnerability Feature}
\label{subsec:vul-feat}
{
Previous research has used examples from the SARD dataset and real-world samples to illustrate how vulnerabilities manifest in software source code\cite{cheng2021deepwukong, chakraborty2021deep, li2021sysevr, fu2022linevul}. We observed some patterns in samples tagged as vulnerable in both these illustrations and existing SVD datasets. Upon further manual investigation, we hypothesized that these patterns often characterize the vulnerability, meaning that the existence of the pattern is directly responsible for the label of the sample in the dataset. To assess the hypotheses, we formally defined these patterns as vulnerability features and how the existence of a feature can contribute to the sample's label (we call it a feature label). To test the accuracy of our feature definitions and their associated labels, we applied static analysis to detect the existence of a feature in a sample. Once we detected a feature, we checked whether the label of the sample and the feature matched. We present the accuracy of our definitions in the results section. For this work, we defined four vulnerability features. In the table below, we present the relevance of each feature on the sample's label and how the label should or should not change when the feature is removed from the sample. We will define the four vulnerability features with examples for the rest of the section.\\
% It is worth noting that specific model architectures utilize their strengths to learn specific types of features. Therefore, assuming that every model architecture should learn all vulnerability features is unfair. Thus, although we will formalize a set $\displaystyle S$ of Vulnerability Features, a feature $\displaystyle S_{i}$ will only be tested if previous literature establishes that the model architecture will learn $\displaystyle S_{i}$. This approach is a fairer assessment of the VDT than trying all of our features. We will define the four vulnerability features with examples for the rest of the section.\\
\textbf{Equality of Definition-Use:} We observed the pattern associated with this feature in many examples of buffer overflow and underflow vulnerabilities. We observed that these examples are fixed by matching the usage in sensitive API calls to the definitions of the variables. Listing \ref{lst:eq_def_use} illustrates this pattern. In lines 5 and 11 of the vulnerable sample in Listing \ref{lst:eq_def_use}, we noticed that the size definition in line 5 does not match the use in line 11. However, the two have an exact match in the fixed version of the sample (i.e., the non-vulnerable sample in Listing \ref{lst:eq_def_use}). In the listing, the sensitive API in question is \texttt{memcpy}, and we observed that vulnerable calls to \texttt{memcpy} can be fixed by matching the size definition in line 5 with the use of data length in line 11. Since the pattern involves the observation of equality between definition and use, we formalize it as a vulnerability feature termed "Equality of Definition-Use."
Furthermore, as the introduction of the feature fixes the vulnerable samples, we define that the relevance of the feature is high in non-vulnerable samples. For the same reason, this feature is not prevalent in vulnerable samples, and even if detected, it is unlikely to cause the vulnerability. However, maliciously removing the feature will revert the sample to the vulnerable version before the fix.\\
\textbf{Equality of Allocation-Deallocation:} This pattern occurs mostly in Use After Free vulnerabilities. When inspecting the Use After Free vulnerabilities, we observed that, just like the definition suggests, these vulnerabilities occur whenever a variable goes through the following control flow: first, a definition via \texttt{malloc} or \texttt{alloca}, then a use in the \texttt{free} function and afterward a use in any context. Listing \ref{lst:eq_alloc_free_after_free} illustrates this property with three samples, one vulnerable and two non-vulnerable. In the vulnerable sample, the variable \texttt{data} was allocated in line 3 and deallocated in line 12. Therefore, once the equality of allocation and deallocation for the variable \texttt{data} occurs, using the variable in line 13 causes a use after free vulnerability. One potential fix involves injecting an inequality of allocation and deallocation before using the variable. Another fix would be removing the use of the variable after equality of allocation and deallocation occurs in the source code. Since the pattern in the vulnerable sample involves a control flow sequence that introduces equality of allocation and deallocation before use, we formalize it as the vulnerability feature, "Equality of Allocation-Deallocation." Additionally, as this feature characterizes the definition of Use After Free vulnerabilities, we further define it as a root cause of vulnerability whenever detected in a vulnerable sample and non-existent in non-vulnerable code samples. By the same logic, if the feature is the only root cause of the vulnerability, upon removing it, the sample's label should change to "non-vulnerable."\\
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Size Overflow},
                label=lst:overflow_size,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/overflow_size.cpp}
\end{minipage}

There is also \\
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Pointer Overflow},
                label=lst:overflow_pointer,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/overflow_pointer.cpp}
\end{minipage}
\textbf{Relevant\saad{Boundary-checking?} Literal Values:} In software vulnerability datasets, we observed that some literals are meaningful in a generalized context, while others are in a specific context. We consider the context-specific meaningful literals as irrelevant features for the task of SVD for two reasons: 1) they are primarily meaningful by accidentally introducing other vulnerability features, and 2) context-specific literals are often meaningless in unseen real-world software source code. On the other hand, we formalize the context-free meaningful literals as Relevant Literal Values for the task of SVD since they are consistent across all projects and datasets. We will inspect buffer underwrite vulnerabilities to illustrate why some literals are universally relevant for this type of vulnerability. In the vulnerable example (Listing \ref{lst:rel_lit}) of such vulnerabilities, we observe that the vulnerability manifests due to insufficient condition-checking in line 4.

%~\tuan{Actually, I think the reasonable fix should be swapping line 12 and 13 in Listing 3. Two proposed fixes in Listing 4 and 5 both have drawbacks. In listing 4, by removing the line $free(data)$ will fix the use-after-free bug but it also causes memory leak. In list 5, by removing the $printIntLine(data[0])$ is not fully reasonable as a statement was put there by developer for specific purpose (e.g., printing values to log file for easier debugging). That means fixing the bug by simply removing the statement like that may change the output of the program. [I suggest we should improve the example by swapping lines as mentioned above.]}\\
% ~\tuan{I can't understand what is "general learning" and why "context-specific" literals are irrelevant features}
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Use After Deallocation},
                label=lst:use_after_dealloc,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/use_after_dealloc.cpp}
\end{minipage}

There is also\\
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Use Before Allocation},
                label=lst:use_before_alloc,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/use_before_alloc.cpp}
\end{minipage}
There is also\\
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Free Before Allocation},
                label=lst:free_before_alloc,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/free_before_alloc.cpp}
\end{minipage}
We can check the upper bound of the buffer by the "Equality of Definition-Use" property described earlier. However, the lower bound should be checked by one of two generally meaningful literal values for checking lower bounds, $\displaystyle 0$ and $\displaystyle -1$. Therefore, comparisons with $\displaystyle 0$ and $\displaystyle -1$ are often used to fix buffer underwrite vulnerabilities. Thus, condition-checking between an array indexing variable and these relevant literals often contributes to the sample's label for non-vulnerable samples.
Similarly, since these comparisons actively prevent out-of-bounds array access, their existence in vulnerable samples does not contribute to the manifestation of vulnerability. However, removing this feature introduces the risk of an out-of-bounds array access. Therefore, a non-vulnerable sample's label should change to vulnerable upon removing the feature.
We also consider $\displaystyle NULL$ and $\displaystyle 1$ as relevant literal values since the former is widely used for null pointer checking and the latter as a truth value.\\
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Numeric Literals},
                label=lst:lit_numeric,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/lit_numeric.cpp}
\end{minipage}
There is also\\
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Object Literals},
                label=lst:lit_object,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/lit_object.cpp}
\end{minipage}
\textbf{Sensitive APIs:} DL-based VDTs that make vulnerability predictions on program slices have listed and used various library functions/APIs as points of interest in the source code to generate program slices from the sample~\cite{li2018vuldeepecker, li2021sysevr, cheng2021deepwukong}. These functions are chosen based on their prevalence and relevance to the manifestation of the vulnerability. Our experiments only consider a small subset of the previously listed APIs directly involved in the vulnerability. We choose this subset based on the transparency of their impact on the vulnerability.
The functions we consider to be relevant are: \texttt{memcpy}, \texttt{strncpy}, \texttt{strcpy}, \texttt{wcsncpy}, \texttt{memset}, \texttt{wmemset}, \texttt{getch}, \texttt{fgets}, \texttt{gets}, \texttt{getchar}, \texttt{fgetc}. We can illustrate this feature with Listings \ref{lst:eq_def_use} and \ref{lst:sensi_write}.
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Write API},
                label=lst:sensi_write,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/sensi_write.cpp}
\end{minipage}

There is also\\
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Read API},
                label=lst:sensi_read,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/sensi_read.cpp}
\end{minipage}
One potential fix to the vulnerability shown in Listing \ref{lst:eq_def_use} would be to replace the function call to the sensitive API \texttt{memcpy} at line 11 with a harmless function call (Listing \ref{lst:sensi_write}).\\
It is worth noting that simply the existence of these APIs does nothing for non-vulnerable samples, as researchers study them primarily for their potential to cause vulnerabilities instead of fixing them. However, if a sensitive API exists in a vulnerable sample, it could be the root cause behind the sample's label or irrelevant in causing the vulnerability. Therefore, it is essential to determine the relevance of the sensitive API for the sample's vulnerability. Since the relevance depends on the sample itself, the effect of removing the feature varies accordingly. If the relevance of a sensitive API is high on a vulnerable sample, then removing the feature should change the sample's label to non-vulnerable. Otherwise, the label should remain unchanged.
% ~\tuan{actually the model doesn't know what is inside the function which we considered as harmless. Thus, expecting its prediction to be changed from vul to non-vul is not reasonable}.
% \tuan{Another thing, as a reader, after going through 4 vulnerability features listed, I feel like you are focusing on only memory-related vulnerability (def-use, alloc bug) instead of general vulnerability}
% \textbf{Condition Comprehensiveness:} This is a compound vulnerability feature since it primarily consists of two or more prior features described. We can refer to Listings \ref{lst:rel_literals_vul}, \ref{lst:rel_literals_nonvul1} and \ref{lst:rel_literals_nonvul2} to expand further on the idea behind the feature. We can characterize the vulnerability observed and their fixes by compounding the "Equality of Definition-Use" and the "Relevant Literal Values" features described above. We observed that a lot of insufficient condition-checking in \texttt{if} statements that cause vulnerabilities can be characterized by a compound of other relevant features we described earlier.\\
}
\subsection{Model Specific Challenges}
\label{subsec:model-challenges}
{
Most SOTA VDTs either use a graph-based Neural Network (NN) architecture or a token-based NN architecture for SVD. These architectures are chosen based on their unique strengths and how they can contribute to learning specific source code features. For example, the rationale behind token-based approaches is that software source code semantics can be represented similarly to natural language(add citation). As for Graph-based approaches, research has discovered that when software source code is represented in a graph format and later fed to a Graph-based Neural Network, the NN can learn different semantic dependencies through their knowledge of data and control edges that token-based approaches cannot learn. However, the NN models face several model-specific challenges~\cite{chakraborty2021deep}, which may hamper the technique's effectiveness. In order to reliably detect vulnerabilities in software source code using these underlying models, it is crucial to ensure that the techniques address these challenges when preprocessing the samples.
% ~\tuan{clarify about [build what?]}
In this paper, we also evaluate how adequately the VDTs address the model-specific challenges by generating source code transformations. However, before we can discuss how to evaluate the VDT's handling of the challenges, we first need to discuss the challenges and how they can affect the learning of the NN model. Therefore, for the rest of the section, we will describe the model-specific challenges and their impact on learning features from source code samples.\\
\textbf{Token-Based Approaches:} Token-based approaches consider software source code as a sequence of tokens usually separated by spaces and language-specific symbols(e.g., semi-colon, colon, interrogation point). However, token-based approaches have to deal with particular challenges that impact their comprehension of the binary classification task they are trying to solve (in this case, vulnerability detection) and, thus, their performance. These challenges include but are not limited to:
\begin{IEEEitemize}
    \item \textbf{Token Relevance:} Token-based approaches often learn the frequency and co-occurrence of tokens in vulnerable and non-vulnerable samples and base their prediction on such information. However, some tokens are irrelevant to the manifestation of vulnerability in a sample. For example, tokens like empty spaces and indentations do not contribute to how a malicious entity can exploit a piece of code. Therefore, if the preprocessing of the samples before training and testing is inadequate, there is a risk of learning such irrelevant information from the dataset.
    \item \textbf{Project-Specific Vocabulary:} Since token-based approaches rely on the prevalence of tokens in samples to make their predictions, they have to ensure they are not learning about the frequency of tokens that appear only in a project-specific context. This is an important factor to consider because project-specific tokens do not generalize how vulnerabilities manifest in software source code, and these approaches can only make predictions based on the tokens. Therefore, unless the preprocessing step involves generalizing the information obtained from the project-specific tokens, the VDT's prediction will not be consistent across unseen projects.
\end{IEEEitemize}
\textbf{Graph-Based Approaches:} Graph-based approaches represent software source code as graphs containing different semantic dependencies in graph edges~\cite{chakraborty2021deep, zhou2019devign}. They use the model's ability to learn about different syntactic and semantic edges in the graph representation to reason about samples in a vulnerability dataset. However, although graph-based approaches can avoid some of the challenges faced by token-based approaches, they have a different set of challenges that they must address to detect vulnerability in code reliably. Some of these challenges are:
\begin{minipage}{\linewidth}
  \centering
  \begin{minipage}{0.4\linewidth}
      \begin{figure}[H]
          \includegraphics[width=\linewidth]{figures/eq_def_use_vul.png}
          \caption{Vulnerable PDG}
          \label{fig:vul_pdg}
      \end{figure}
  \end{minipage}
  \hspace{0.05\linewidth}
  \begin{minipage}{0.4\linewidth}
      \begin{figure}[H]
          \includegraphics[width=\linewidth]{figures/eq_def_use_vul.png}
          \caption{Non-Vulnerable PDG}
          \label{fig:nonvul_pdg}
      \end{figure}
  \end{minipage}
\end{minipage}
\begin{IEEEitemize}
    \item \textbf{Edge Property:} One rationale behind graph-based approaches is their ability to learn different syntactic and semantic dependencies through understanding graph edges. However, we still need precise details on what information about the edges the VDT is using for vulnerability prediction. Unfortunately, the current state of research does not provide that information. Despite that, it is still essential to understand the depth of the VDT's comprehension of the graph edges and test if they are learning irrelevant edge information. For example, figures \ref{fig:vul_pdg} and \ref{fig:nonvul_pdg} illustrate the Program Dependence Graph of the vulnerable and non-vulnerable samples in Listing \ref{lst:eq_def_use}. The black edges represent data dependency, and the blue represents control dependency. Here, the two PDGs look identical regarding the edges that connect the line numbers; however, the edge connecting lines 5 and 11 is vulnerable in the PDG of the vulnerable sample (red edge), but the same edge is non-vulnerable in the PDG of the non-vulnerable sample (green edge\saad{it's not green in the figure}). Upon inspecting Listing \ref{lst:eq_def_use}, we see that the contents of lines 5 and 11 have the "Equality of Definition-Use" property in the non-vulnerable version. In contrast, the vulnerable version violates the property. Therefore, the same edge can be vulnerable or non-vulnerable depending on the contents of the two connected nodes. In such cases, it is not sufficient to learn only the existence of the edge.
    \item  \textbf{Path Coverage Information:} Current SVD datasets contain information about the static properties of the source code samples, and graph-based approaches extract this information when generating the graph representation of the source code. However, current public vulnerability datasets do not incorporate runtime information like path coverage during curation, and yet, sometimes, it may accidentally show up in a sample. When that happens, it is important to base the prediction on something other than that information (e.g., a vulnerability feature) since there has been no effort to generalize its effect on vulnerability across all samples. This case is illustrated in Listing \ref{lst:path_cov}. In the vulnerable sample, the vulnerability occurs due to the violation of the "Equality of Definition-Use" property in the sample. However, the vulnerability is fixed by first enforcing the "Equality of Definition-Use" property and later changing the condition inside the \texttt{if} statement to become unsatisfiable, leading to the execution of the code in the \texttt{else} block. Samples like this accidentally provide runtime information, which should not be the basis of vulnerability prediction until there is a way to generalize its effect on vulnerability across all samples that contain the information. In situations like this, the prediction should be made based on information like "Equality of Definition-Use" since it has a generalized impact on causing vulnerability in samples that contain the property.
\end{IEEEitemize}
\noindent\begin{minipage}{.5\textwidth}
    \lstinputlisting[language=C++, 
                    caption={Path Coverage Information},
                    label=lst:path_cov,
                    mathescape,
                    escapechar=@,
                    xleftmargin=0cm,
                    xrightmargin=0cm]
                    {code/path_cov.cpp}
    \end{minipage}


% Token-based approaches to SVD can suffer from token proximity issues,
% ~\tuan{this issue is not listed on the weaknesses of Token-Based Approaches (previous paragraph)}
% and to address it, Graph-Based methods rely on the model's ability to learn data and control edges~\cite{chakraborty2021deep, zhou2019devign}. However, simply learning the existence of a data/control edge between two nodes in a code representation graph is not sufficient to learn the manifestation of the vulnerability since the same edge can exist in vulnerable and non-vulnerable samples depending on the property of the edge as well as the two connecting nodes.
% ~\tuan{the reasoning is not clearly explained, maybe giving a figure of code example could help}
% For example, "Equality of Definition-Use" and "Inequality of Allocation-Deallocation" are properties that contribute more to the vulnerability than a data or control edge.
% ~\tuan{I see that the edges connecting between nodes does realize the def-use relationship, and this contributes to detect the vulnerability. It's not suitable to compare "more" or "less" here.}
% Therefore, such techniques must learn those properties to predict the graph correctly. Furthermore, since graph-based techniques generate the graph representation of software source code via various static analysis techniques, they don't have access to runtime properties of the program state, meaning they should not be learning program-state properties such as condition satisfiability or input-dependent path coverage. Instead, their prediction should depend on the full path coverage of the software source (i.e., assume that all paths are reachable).
% ~\adriana{Why?}.
% ~\tuan{I do have the same feeling as Adriana's. I don't understand why you are mentioning the program-state properties here.} 
}
}

==> sections/definitions.tex <==
\section{Second Section}
\label{sec:definitions}
{
% \textbf{We want to enable a systematic study of current and future vulnerability detection techniques.}\\
To facilitate continuous improvement in detecting vulnerabilities in software source code, it is essential to first enable systematic studies of current and future techniques.
% \textbf{Such a systematic study is predicated on understanding the features these techniques learn.}\\
However, such studies and the resulting improvements are contingent upon obtaining a reasonable understanding of what features are important for comprehending and recognizing vulnerabilities (Vulnerability Features hereafter) and which ones do not provide any information about the vulnerability despite having a strong correlation with the target labels (Spurious Features hereafter). Since the robustness and general applicability of vulnerability detection techniques (or any detection technique) involve recognizing the right features and ignoring the wrong ones, we hypothesize that the existing techniques have been so poor on those fronts because they are not only failing to learn the Vulnerability Features but also learning Spurious Features.\\
% \textbf{Introduce the concept of code property as the linchpin of this.}\\
Before we study the features of code, we need to represent the samples in the dataset (in this case, source code) in a structure that allows meaningful analysis and pattern detection. The Code Property Graph (CPG) is popular in the community as a reasonable basis for representing and detecting various properties of source code. A CPG is a property graph constructed from the Abstract Syntax Tree (AST), Control Flow Graph (CFG), and Program Dependence Graph (PDG) of source code that combines their labeling and property functions, and it allows expression and analysis of different kinds of programming patterns especially for well-known types of vulnerabilities\cite{yamaguchi2014modeling}. Therefore, we used the CPG as a basis to express features of code (Code Features hereafter).\\
% \\\textbf{This leads to the concept of vulnerability features.}\\
% \\\textbf{It also leads to our hypothesis that someone could be learning the wrong things – spurious features}\\
% \\\textbf{To do this we also need to consider a wide range of vulnerabilities – hence SARD (this is where the above comments come in)}\\
To understand which features of the samples in a vulnerability dataset the curators intend for a tool to learn, we analyzed the most recent and popular vulnerability datasets: SARD\cite{sard}, FFmpeg+Qemu\cite{zhou2019devign}, Dapper\cite{russell2018automated} and BigVul\cite{fan2020ac}. However, only the SARD dataset met our requirements for the latter analyses for the following reasons:
\begin{minipage}{\linewidth}
  \centering
  \begin{minipage}{0.4\linewidth}
      \begin{figure}[H]
          \includegraphics[width=\linewidth]{figures/vul_sample.png}
          \caption{Vulnerable Sample}
          \label{fig:vul_sample}
      \end{figure}
  \end{minipage}
  \hspace{0.05\linewidth}
  \begin{minipage}{0.4\linewidth}
      \begin{figure}[H]
          \includegraphics[width=\linewidth]{figures/nonvul_sample.png}
          \caption{Non-Vulnerable Sample}
          \label{fig:nonvul_sample}
      \end{figure}
  \end{minipage}
\end{minipage}
\begin{IEEEitemize}
    \item Only the SARD dataset involves generating samples highlighting how a vulnerability manifests itself in the source code and how we can fix it by applying a minimal change in the source code during curation. The curators achieve this by carefully annotating the source code in critical points, and these annotations describe how the vulnerability manifests itself in the vulnerable sample (Figure \ref{fig:vul_sample}) and what changes we can apply to fix them in the non-vulnerable sample (Figure \ref{fig:nonvul_sample}). The lack of this vital information in other datasets means the process of identifying features and their relevance in causing vulnerability cannot be reliably verified, making them unsuitable.
	\item The SARD dataset is the oldest and largest vulnerability dataset, which is continuously growing and is very prominently supported by researchers, open-source developers, and the National Institute of Standards and Technology.
\end{IEEEitemize}
We studied the dataset by first identifying the most frequent vulnerabilities. We then manually analyzed their descriptions and corresponding source code lines to understand what parts of the code contributed to the vulnerability. Our goal was to manually convert each unique description into a set of Code Property Graph Rules (CPGRs). On that front, we successfully expressed eight descriptions of vulnerabilities into sets of CPGRs that we used to represent Vulnerability Features.\\
To study Spurious Features, we used the established intuitions from previous literature as a basis for features that influence predictions of Token-based approaches. Additionally, we explored the assumptions made in Graph-Based approaches to identify properties in graph representations of code that exist merely as false correlations. To facilitate consistency, we follow the same representation strategy we used for Vulnerability Features on the Spurious Features (i.e., use sets of CPGRs to express them).\\
Our efforts to express the Vulnerability and Spurious Features led us to propose a taxonomy of Code Features that can be used to express distinguishing characteristics of Vulnerability and Spurious Features as well as find relations between similar features. The taxonomy is illustrated in Figure \ref{tax:code_feat}.
\input{taxonomy/taxonomy}
% For any prediction task, samples in the dataset can contain features that represent the core characteristics defining the prediction task and those that merely exist as a correlation. In the case of vulnerability prediction, the sample source codes in the dataset contain combinations of code properties (defined by Yamaguchi, Fabian, et al.\cite{yamaguchi2014modeling}) that correlate highly with the target label and also characterize the cause of the vulnerability. At the same time, other properties may exist in the samples merely as false correlations that do not contribute towards the vulnerability and how it manifests in the source code. In this paper, we will refer to them collectively as code features. However, we will call those that characterize a vulnerability a vulnerability feature and those that do not a spurious feature (coined by Rahman, Md Mahbubur, et al.\cite{rahman2023towards}).\\
\subsection{Vulnerability Features}
\label{subsec:vul_feat}
{
As described above, Vulnerability Features characterize how a vulnerability manifests in the vulnerable sample. Based on the characteristics provided in the annotated descriptions in the SARD dataset, we can generate a specific combination of code properties to represent the feature. While we encourage the community to extend the vulnerability features, we limit them to only those we could translate into a combination of code properties for this work.
\subsubsection{Overflow Vulnerability}
\label{subsubsec:overflow}
{
According to the SARD dataset's description, a buffer overflow occurs when writing and reading from a buffer if there are discrepancies between the definition of the pointers (definition space hereafter) and their sizes with the used pointers and sizes (use space hereafter). Specifically, an overflow error will occur if the size is larger in the use space than in the definition space or a pointer is larger in the use space than in the definition space. Therefore, we categorize an overflow vulnerability into the following categories:\\
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Size Overflow},
                label=lst:overflow_size,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/overflow_size.cpp}
\end{minipage}
\textbf{Size Overflow:} An overflow vulnerability can manifest if the size in the use space is larger than in the definition space. Listing \ref{lst:overflow_size} illustrates such an occurrence. In lines 5 (definition space) and 11 (use space) of the vulnerable sample, we noticed that the size in the use space does not match the one in the definition space. Since the size in the use space is larger than in the definition space, this causes an overflow error.\\
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Pointer Overflow},
                label=lst:overflow_pointer,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/overflow_pointer.cpp}
\end{minipage}
\textbf{Pointer Overflow:} An overflow vulnerability can also manifest if the pointer in the use space is larger than in the definition space. Like Listing \ref{lst:overflow_size}, Listing \ref{lst:overflow_pointer} also has line 5 as the definition space and line 11 as the use space. The pointer \texttt{data} is larger in the use space than in the definition space, leading to an overflow error.\\
}

\subsubsection{Unauthorized Buffer Use Vulnerability}
\label{subsubsec:unauth_buff_use}
{
The annotations in the SARD dataset describe the manifestation
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Use After Deallocation},
                label=lst:use_after_dealloc,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/use_after_dealloc.cpp}
\end{minipage}
of vulnerabilities that involve using an unauthorized buffer, as when a use space occurs involving a buffer that has already been freed. We extended the manifestation description to incorporate vulnerabilities involving a use before allocation where we encounter the buffer in a use space before encountering it in a definition allocation space.
This feature characterizes two types of vulnerability manifestations:\\
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Use Before Allocation},
                label=lst:use_before_alloc,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/use_before_alloc.cpp}
\end{minipage}
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Free Before Allocation},
                label=lst:free_before_alloc,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/free_before_alloc.cpp}
\end{minipage}
\textbf{Use After Deallocation:} When a use space encounter occurs after a deallocation definition space, it allows using an unauthorized buffer. This scenario effectively depicts the case where a buffer gets allocated and then properly deallocated, but the buffer later appears in a use space.
To illustrate, the vulnerable sample in Listing \ref{lst:use_after_dealloc} contains a use space in Line 13 where the buffer \texttt{data} has been deallocated in Line 12 after initially being allocated in the definition space in Line 3. The fixes for this type of vulnerability involve either moving the use space before the deallocation definition space (first non-vulnerable sample in Listing \ref{lst:use_after_dealloc}) or removing the use space altogether (second non-vulnerable sample in Listing \ref{lst:use_after_dealloc}).\\
\textbf{Use Before Allocation:} When a use space encounter occurs before an allocation definition space, that also manifests a use of an unauthorized buffer. To further elaborate, this scenario can occur in two ways: Either when we encounter a buffer in a use space (Line 3 in Listing \ref{lst:use_before_alloc}) before we ever encounter it in an allocation definition space (Line 4 in Listing \ref{lst:use_before_alloc}) or
when we encounter a buffer in a deallocation definition space (Line 3 in Listing \ref{lst:free_before_alloc}) before we encounter it in an allocation definition space (Line 4 in Listing \ref{lst:free_before_alloc}). The fixes are similar to the ones in Listing \ref{lst:use_after_dealloc}.\\
}

\subsubsection{Buffer Underwrite Vulnerability}
\label{subsubsec:buff_undrw}
{
The curators of the SARD dataset manifested buffer underwrite vulnerabilities by accessing an unbound location of an array. They generated the fix by simply doing a boundary check for the index. We can categorize this boundary checking into the following:\\
\textbf{Numeric Literals:} These numeric literals are used for checking the lower bound of an array index. Typically, 0 and -1 fall under this category. Listing \ref{lst:lit_numeric} illustrates this property. In Line 4 of the vulnerable sample, the index variable data only goes through an upper boundary check but not a lower one, allowing buffer underwrite to occur. The curators generate the fix by adding a "greater than" comparison with -1 or a "greater than equal to" comparison with 0 as a conjunction.\\
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Numeric Literals},
                label=lst:lit_numeric,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/lit_numeric.cpp}
\end{minipage}
\textbf{Object Literals:} The literal used for comparing objects is \texttt{NULL}, which is used in fixes that check if a pointer is valid. Listing \ref{lst:lit_object} depicts the use of object literals. Lines 2 and 3 of the vulnerable sample use the \texttt{buf} object without checking its validity. The curators of the SARD dataset generated the fix by adding a comparison with the object literal \texttt{NULL}. (Line 2 of Listing \ref{lst:lit_object}).\\
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Object Literals},
                label=lst:lit_object,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/lit_object.cpp}
\end{minipage}
}
\subsubsection{Sensitive Read/Write Vulnerability}
\label{subsubsec:sensi_w_r}
{
SVDTs that extract program slices from code snippets select their points of interest, and often, these points of interest refer to points of failure in the code if an attacker exploits the vulnerability.
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Write API},
                label=lst:sensi_write,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/sensi_write.cpp}
\end{minipage}
Studies have further revealed that these points of failure frequently contain calls to several commonly occurring library APIs and have listed them as sensitive APIs in the context of vulnerable code snippets. For this work, we focus on the most widely occurring sensitive APIs and categorize them into two categories: Read APIs and Write APIs.\\
\textbf{Write APIs:} The functionality of these sensitive APIs involves writing data to a buffer. APIs in this category include: \texttt{memcpy}, \texttt{strncpy}, \texttt{strcpy}, \texttt{wcsncpy}, \texttt{memset}, and \texttt{wmemset}. Listing \ref{lst:sensi_write} illustrates this property. Here, the vulnerable code sample contains an API call to the library function, \texttt{memcpy} and one potential way to prevent exploiting the vulnerability would be to replace the function call to the sensitive API with a harmless function call.\\
\textbf{Read APIs:} The functionality of these sensitive APIs involves reading user data from a source and storing them in a buffer. APIs in this category include: \texttt{fgets}, \texttt{getch}, \texttt{gets}, \texttt{getchar}, and \texttt{fgetc}. Upon closer inspection of Listing \ref{lst:sensi_read}, we observe that the point of failure in the vulnerable sample is in line 11, which is a function call to \texttt{fgets}. To avoid exploiting this vulnerability, we can change the function call to a harmless function, as shown in the non-vulnerable sample.\\
\noindent\begin{minipage}{.5\textwidth}
\lstinputlisting[language=C++, 
                caption={Read API},
                label=lst:sensi_read,
                mathescape,
                escapechar=@,
                xleftmargin=0cm,
                xrightmargin=0cm]
                {code/sensi_read.cpp}
\end{minipage}
}

}
\subsection{Spurious Features}
\label{subsec:spu_feat}
{
Existing state-of-the-art SVDTs either use a graph-based Neural Network or a token-based one \cite{fu2022linevul, li2021sysevr, chakraborty2021deep, cheng2021deepwukong}. The authors choose these architectures intending to utilize the architecture's strengths to make effective predictions. However, like any other dataset for prediction tasks, source code samples may contain features that reveal their label simply as a correlation. If such features strongly influence the predictions of a binary classification technique, then it loses practical applicability. Rahman, Md Mahbubur, et al\cite{rahman2023towards}. coined the term Spurious Features to denote such features in vulnerability datasets. Previous studies have established some Spurious Features for token-based approaches based on intuitions and background knowledge of the problem \cite{rahman2023towards, risse2023limits}. In our taxonomy, we categorize these spurious features, provide a new feature for token-based approaches, and introduce spurious features for graph-based approaches. It is important to make this separation because the two approaches render them resistant to the spurious features of the other due to how they represent the samples.
}
}

==> tables/fp_fr_for_4_tools.tex <==
\begin{table}[!h]
        \centering
        
\caption{SySeVR}
\begin{tabular}{|p{0.30\linewidth}|p{0.25\linewidth}|p{0.25\linewidth}|}
\hline 
 \textbf{Feature Name} & \textbf{FP Success Rate} & \textbf{FR Success Rate} \\
\hline 
 incorr\_calc\_buff\_size & 0 & 100 \\
\hline 
 buff\_access\_src\_size & 0 & 100 \\
\hline 
 off\_by\_one & 3.07692307692308 & 79.3650793650794 \\
\hline 
 buff\_overread & 4.10958904109589 & 82.8571428571429 \\
\hline 
 double\_free & 35.7142857142857 & 8.33333333333333 \\
\hline 
 use\_after\_free & 6.14035087719298 & 55.6962025316456 \\
\hline 
 buff\_underwrite & 5.56844547563805 & 91.421568627451 \\
\hline 
 buff\_underread & 1.28205128205128 & 97.9166666666667 \\
\hline 
 sensi\_read & 0 & 0 \\
\hline 
 sensi\_write & 0& 81.6326530612245 \\
 \hline
\end{tabular}
        
\end{table}

\begin{table}[!h]
        \centering
        
\caption{DeepWukong}
\begin{tabular}{|p{0.30\linewidth}|p{0.25\linewidth}|p{0.25\linewidth}|}
\hline 
 \textbf{Feature Name} & \textbf{FP Success Rate} & \textbf{FR Success Rate} \\
\hline 
 incorr\_calc\_buff\_size & 0.670578373847443
 & 67.8670360110803 \\
\hline 
 buff\_access\_src\_size & 0.752823086574655
 & 52.5 \\
\hline 
 off\_by\_one & 0.373134328358209 & 94.7019867549669
 \\
\hline 
 buff\_overread & 0.032414910858995 & 89.7350993377484 \\
\hline 
 double\_free & 0 & 100 \\
\hline 
 use\_after\_free & 0 & 98.8095238095238 \\
\hline 
 buff\_underwrite & 8.54653633659159 & 65.0824272185198 \\
\hline 
 buff\_underread & 0.714916151809356 & 94.1235059760956 \\
\hline 
 sensi\_read & 0 & 0 \\
\hline 
 sensi\_write & 1.27306273062731& 56.0743211052882 \\
 \hline
\end{tabular}
        
\end{table}

\begin{table}[!h]
        \centering
        
\caption{LineVul}
\begin{tabular}{|p{0.30\linewidth}|p{0.25\linewidth}|p{0.25\linewidth}|}
\hline 
 \textbf{Feature Name} & \textbf{FP Success Rate} & \textbf{FR Success Rate} \\
\hline 
 incorr\_calc\_buff\_size & 0 & 100 \\
\hline 
 buff\_access\_src\_size & 0 & 100 \\
\hline 
 off\_by\_one & 0 & 100 \\
\hline 
 buff\_overread & 0 & 100 \\
\hline 
 double\_free & 0 & 100 \\
\hline 
 use\_after\_free & 0 & 100 \\
\hline 
 buff\_underwrite & 0 & 100 \\
\hline 
 buff\_underread & 0 & 100 \\
\hline 
 sensi\_read & 0 & 100 \\
\hline 
 sensi\_write & 0 & 100 \\
 \hline
\end{tabular}

        
\end{table}

\begin{table}[!h]
        \centering
        
\caption{ReVeal}
\begin{tabular}{|p{0.30\linewidth}|p{0.25\linewidth}|p{0.25\linewidth}|}
\hline 
 \textbf{Feature Name} & \textbf{FP Success Rate} & \textbf{FR Success Rate} \\
\hline 
incorr\_calc\_buff\_siz & 0.0 & 100.0 \\
\hline 
buff\_access\_src\_size & 0.0 & 100.0 \\
\hline 
off\_by\_one & 1.8229166666666667 & 80.48780487804879 \\
\hline 
buff\_overread & 0.5671902268760907 & 95.0413223140496 \\
\hline 
double\_free & 35.714285714285715 & 69.04761904761905 \\
\hline 
use\_after\_free & 5.769230769230769 & 64.34108527131784 \\
\hline 
buff\_underwrite & 1.477832512315271 & 94.77163461538461 \\
\hline 
buff\_underread & 1.1336227689339122 & 95.28985507246377 \\
\hline 
sensi\_read & 0.0 & 0.0 \\
\hline 
sensi\_write & 0.0 & 0.0 \\
 \hline
\end{tabular}
        
\end{table}



==> taxonomy/taxonomy.tex <==
% \begin{minipage}{0.6\linewidth}
  % \centering
  % \begin{minipage}{\linewidth}
      \begin{figure}[htbp]
        \begin{forest}
              for tree={
                font=\footnotesize,
                grow'=0,
                child anchor=west,
                parent anchor=south,
                anchor=west,
                calign=first,
                % inner xsep=0pt,
                inner ysep=-2pt,
                outer ysep=0pt,
                forked edges,
                edge path={
                    \noexpand\path [draw, \forestoption{edge}]
                    (!u.south west) +(4pt,0) |- (.child anchor) \forestoption{edge label};
                },
                before typesetting nodes={
                    if n=1
                    {insert before={[,phantom]}}
                    {}
                },
                fit=band,
                before computing xy={l=8pt},
              }  
            [
            Code Features
                        [Vulnerability Features
                            [Overflow
                                [Incorrect Calculation of Buffer Size]
                                [Buffer Access Using Size of Source Buffer]
                                [Buffer Access Using Size of Destination Buffer]
                                [Off-by-one Error]
                            ]
                            [Deallocated Buffer Use
                                [Use-After-Free]
                                [Double-Free]
                            ]
                            [Numeric Range Comparison Without Minimum Check
                                [Buffer Underwrite]
                                [Buffer Under-read]
                            ]
                            [Sensitive API Call
                                [Read API]
                                [Write API]
                            ]
                        ]
                        [Spurious Features
                            [
                                Custom Coding Conventions
                                [Token-based
                                    [Identifier Names
                                    ]
                                    [Code Formatting
                                    ]
                                ]
                                [Graph-based
                                    [Edge Set]
                                    [Node Set]
                                ]
                            ]
                        ]
            ]
            \end{forest}
          % \captionsetup{width=\linewidth, format=hang}
          \caption{Taxonomy of Code Features}
          \label{tax:code_feat}
      \end{figure}
%   \end{minipage}
% \end{minipage}

==> transformation_rules/dealloc/double_free.tex <==
$\displaystyle \exists v\in V':\exists x\in DA_{b} :\exists y\in DA_{b} ,( edge( x,y) \in E) \land ( \lambda ( x,y) =``POST\_DOM")$\\
\textbf{LP Transformation Formula:} The key characteristics of the CPG rule are the postdominance relationship between two nodes $\displaystyle u\&v$ that deallocate the same buffer $\displaystyle b$ and the absence of postdominance between $\displaystyle u$ and any allocation node, and the LP transformations should ensure this property holds even after the transformation. One way to transform the code would be to add an allocation node, $\displaystyle a_{n}$, where $\displaystyle a_{n}$ postdominates both $\displaystyle u\&v$. Doing this will facilitate an illusion of a fix, but since it maintains the CPG rule for Double-Free errors, the target label of the sample will not change. This is depicted in the formula below:\\
$\displaystyle F_{1}:$ Set of library functions used for allocating heap memory\\
$\displaystyle a_{n}:$ New allocation node\\
$\displaystyle u:$ CPG Node declaring the buffer $\displaystyle b$.
\begin{gather*}
A_{b} :=\{v\in V|\exists u\in V,\ edge( v,u) \in E\\
\land\lambda ( v,u) =``DEF"\land \mu ( u,K=``Symbol") =b\\
\land \mu ( v,K=``type") =``CallExpression"\\
\land \mu ( v,K=``Callee") \in F_{1}\}\\
\mu ( a_{n} ,K=``type") \ :=\ ``CallExpression"\\
\mu ( a_{n} ,K=``Callee") \ :=\ f\in F_{1}\\
u:=\{u\in V|\mu ( u,K=``Symbol") =b\}\\
E_{n} :=E\cup \{edge( a_{n} ,u)\}\\
\lambda ( a_{n} ,u) :=``DEF"\\
Set\ E:=E_{n}\\
A_{b} ':=A_{b} \cup \{a_{n}\}\\
Set\ A_{b} :=A_{b} '\\
\forall x\in DA_{b} \Longrightarrow\\
E_{n} :=E\cup \{edge( a_{n} ,x)\}\\
\lambda ( a_{n} ,x) :=``POST\_DOM "\\
Set\ E:=E_{n}
\end{gather*}
\textbf{LI Transformation Formula:} The fixes for Double-Free errors in the SARD dataset involve removing the postdominated deallocation node $\displaystyle u$ which can be depicted by the formula below:\\
$\displaystyle DA_{b}^{p} :$ Set of de-allocation CPG nodes that are postdominated by another de-allocation node.\\
\begin{gather*}
DA_{b}^{p} :=\{x\in DA_{b} |\exists y\in DA_{b} ,( edge( y,x) \in E)\\
\land ( \lambda ( y,x) =``POST\_DOM")\}\\
V':=V-DA_{b}^{p}\\
E':=E-\left\{( x,y) \in E|x\in DA_{b}^{p} \lor y\in DA_{b}^{p}\right\}\\
Set V:=V'\\
Set E:=E'\\
Set DA_{b} :=DA_{b} -DA_{b}^{p}
\end{gather*}

==> transformation_rules/dealloc/use_after_free.tex <==
$\displaystyle \exists v\in V':\exists x\in RD_{b}:\exists y\in DA_{b} ,( edge( x,y) \in E) \land ( \lambda ( x,y) =``POST\_DOM")$\\
\textbf{LP Transformation Formula:} Use-After-Free errors are characterized by a deallocation $\displaystyle u$ of buffer $\displaystyle b$ that is postdominated by a use $\displaystyle v$ of $\displaystyle b$ where $\displaystyle v$ does not postdominate an allocation $\displaystyle a_{n}$ of $\displaystyle b$ if $\displaystyle u$ does not postdominate $\displaystyle a_{n}$. To generate LP transformations for Use-After-Free errors, we follow a similar strategy to what we used for Double-Free errors and introduce a new allocation node $\displaystyle a_{n}$ for buffer $\displaystyle b$ in the CPG while maintaining properties mentioned in the CPG rule. This is depicted in the formula below:
\begin{gather*}
\forall x\in RD_{b} \Longrightarrow\\
E_{n} :=E\cup \{edge( a_{n} ,x)\}\\
\lambda ( a_{n} ,x) :=``POST\_DOM "\\
Set\ E:=E_{n}
\end{gather*}
\textbf{LI Transformation Formula:} The samples in the SARD dataset fix Use-After-Free by reordering the nodes in the CPG that manifest the postdominance relationship between $\displaystyle u\&v$. This motivates the formula below that we used to generate LI transformations for this vulnerability:
\begin{gather*}    
\forall v\in DA_{b}^{p} \Longrightarrow \\
E_{v} :=\{edge( x,y) \in E|y=v\\
\land \lambda ( x,y) =``POST\_DOM"\land x\in RD_{b}\}\\
\forall e\in E'\Longrightarrow \\
e':=edge( y,x)\\
\lambda ( y,x) :=``POST\_DOM"\\
E_{N} :=( E-\{e\}) \cup \{e'\}\\
Set\ E:=E_{n}\\
\end{gather*}

==> transformation_rules/num_range/underwrite.tex <==
$\displaystyle C_{idx}^{v} =\phi $\\
\textbf{LP Transformation Formula:} The key property of this vulnerability is that a buffer is accessed for a read or write operation with an index value without checking the lower bound of the index value (i.e., not checking if the index has a negative value). Since this vulnerability is centered around the control nodes for the index variable, our transformations focus on altering the control dependence of the index variable. To retain the target label of the sample after altering the control dependence, we need to ensure that the transformation does not violate the property $\displaystyle C_{idx}^{v} =\phi $\ of the CPG rule. We achieve this with the formula below:\\
$\displaystyle c_{n}:$ New Control Node
\begin{gather*}    
\mu ( c_{n} ,K=``type") :=``RelationalExpression"\\
\mu ( c_{n} ,K=``operator") :=``\geqslant "\\
\mu ( c_{n} ,K=``Identifier") :=idx\\
\mu ( c_{n} ,K=``MultiplicativeExpression") :=2\times ( -1) \times l;
\end{gather*}
Where,
\begin{gather*}    
l:=max( L_{b})\\
e':edge( c_{n} ,v)\\
\lambda ( c_{n} ,v) :=``CONTROLS"\\
E_{N} :=E\cup \{e'\}\\
V_{n} :=V\cup \{c_{n}\}\\
Set\ V:=V_{n}\\
Set\ E:=E_{n}
\end{gather*}
\textbf{LI Transformation Formula:} The samples in the SARD dataset fix this vulnerability by simply adding a ``$\displaystyle \geqslant $" comparison between the index and \texttt{0}. Therefore, we generate LI transformations for this vulnerability using the following formula:\\

1. $\displaystyle \mu ( c_{n} ,K=``PrimaryExpression") :=0$\\

Following a similar philosophy to the one mentioned above, we develop another LI transformation for this feature, where we add a control node with a $\displaystyle  >$ comparison between the index and \texttt{-1}. The formula below depicts this:\\

2. $\displaystyle \mu ( c_{n} ,K=``operator") :=`` >"$\\

$\displaystyle \mu ( c_{n} ,K=``PrimaryExpression") :=-1$\\

==> transformation_rules/overflow/off-by-one.tex <==
$\displaystyle \exists v\in V':( l\notin L_{d}) \ \land ( l\in L_{s} ')$; Where,\\
$\displaystyle L_{s} ':$ Buffer lengths for $\displaystyle s$ that are greater than the length of $\displaystyle d$ by one.\\
\textbf{LP Transformation Formula:} This vulnerability is slightly different from the previous ones described above as it is characterized by the programmers' tendency to include the null character,\texttt{`\textbackslash0'} while writing to a buffer. This leads to a source buffer size larger than the destination buffer by exactly one. Therefore, to generate LP transformations, we change the size of the buffer to a size in the source buffer that is larger than the size of the destination buffer by one. To accommodate this change, we first add an increased size value $\displaystyle L_{n}$ to the sizes for the destination buffer $\displaystyle d$. Next, we add a size value $\displaystyle L_{n} + 1$ to the sizes for the source buffer $\displaystyle s$. Lastly, we set the value of $\displaystyle l$ to $\displaystyle L_{n} + 1$. The details of these operations are given below:
\begin{gather*}
L_{n} :=l+I_{0}\\
L_{d} ':=L_{d} \cup \{L_{n}\}\\
Set\ L_{d} :=L_{d} '\\
L_{s} '':=L_{s} \cup \{L_{n} +1\}\\
Set\ L_{s}:=L_{s} ''\\
Set\ l:=L_{n}\\
\end{gather*}
\textbf{LI Transformation Formula:} The curators of the SARD dataset fix this error in the same manner as the Incorrect Calculation of Buffer Size error. Therefore, we use the same formula to generate the Label Inverting transformations described previously.\\

==> transformation_rules/overflow/over_read.tex <==
$\displaystyle \exists v\in V':( l\notin L_{s}) \ \land ( l\in L_{d} ')$\\
\textbf{LP Transformation Formula:} We use a similar transformation strategy as the one we used for ``Buffer Access Using Size of Source Buffer" except that we will focus on holding the property $\displaystyle L_{n} \in L_{d} '$. We do that by adding $\displaystyle L_{n}$ to the list of buffer lengths for the destination buffer $\displaystyle d$. The formula below depicts this operation:
\begin{gather*}    
I:=\{i\ \in \{1,2,3,...,100\} |l+i\notin L_{d} '\}\\
L_{n} :=l+I_{0}\\
L_{d_{n}} :=L_{d} \cup \{L_{n}\}\\
Set\ L_{d} :=L_{d_{n}}\\
Set\ l:=L_{n}
\end{gather*}
\textbf{LI Transformation Formula:} The fixes in the SARD dataset for this vulnerability involves matching the size used in the write operation to the size of the source buffer $\displaystyle s$ which violates the property: $\displaystyle l\notin L_{s}$. Therefore, we use the following formula to generate the LI transformations:
\begin{gather*}
L_{n} :=x\in L_{s}\\
Set \l:=L_{n}
\end{gather*}

==> transformation_rules/overflow/src_size.tex <==
$\displaystyle \exists v\in V':( l\notin L_{d}) \ \land ( l\in L_{s} ')$\\
\textbf{LP Transformation Formula:} To generate Label-preserving transformations for this feature by changing $\displaystyle l$, we need to ensure that the transformation does not violate $\displaystyle l\notin L_{d} \land l\in L'_{s}$. We follow the same formula described above to change the value of $\displaystyle l$ to $\displaystyle L_{n}$. However, for this formula, we need to ensure that the property $\displaystyle L_{n} \in L_{s} '$ holds, and we do that by adding $\displaystyle L_{n}$ to the list of buffer lengths for the source buffer $\displaystyle s$. This is illustrated in the formula below:
\begin{gather*}
I:=\{i\ \in \{1,2,3,...,100\} |l+i\notin L_{s} '\}\\
L_{n} :=l+I_{0}\\
L_{s_{n}} :=L_{s} \cup \{L_{n}\}\\
Set\ L_{s} :=L_{s_{n}}\\    
Set\ l:=L_{n}
\end{gather*}
\textbf{LI Transformation Formula:} The samples in the SARD dataset fix this error the same way as the previous vulnerability (i.e., matching the size used in the write operation with the size of the destination buffer). Therefore, we use the same LI Transformation Formula as before.\\

==> transformation_rules/sensi_read_write/sensi_r_w.tex <==
$\displaystyle \mathcal{L} \cap Y\neq \phi $\\
% \saad{Here, I feel like we need to provide context for the rule we just described. The reader should not have to go back to the previous section to look it up.}
Since this vulnerability focuses on the presence of the sensitive Read/Write APIs in points of failure in the sample, the framework generates transformations by altering the function calls made in those locations.\\
\textbf{FP Transformation Strategy:} To maintain the property of calling a sensitive API in locations causing the failure, the transformation needs to ensure that the function call in such a location is to a different function $\displaystyle f\in F$. This can be achieved by using the following strategy:\\
$\displaystyle f:$ Sensitive API called at node $\displaystyle v$.\\
$\displaystyle F':$ Set of Sensitive APIs that are not called at node $\displaystyle v$.\\
\begin{gather*}
V':=\{v\in V|\mu ( v,K=``type") =``CallExpression"\\
\land \mu ( v,K=``Callee") \in F\land \mu ( v,K=``loc") \in Y\}\\
\forall v\in V'\Longrightarrow\\
f:=\mu ( v,K=``Callee")\\
F':=\{x\in F:x\neq f\}\\
Set\ \mu ( v,K=``Callee") :=x\in F'
\end{gather*}
Although this transformation changes the function call to failure location, it still calls a sensitive API that causes the vulnerability. Therefore, the CPG rule holds even after the transformation and the feature still remains. For a transformation like this, the tools should not change their predictions.\\
\textbf{FR Transformation Strategy:} To generate FR transformations, the framework only needs to ensure that the function call in node $\displaystyle v$ does not involve any function $\displaystyle x\in F$ in the transformed samples. It achieves this by the following strategy:\\
$\displaystyle \mu ( v,K=``Callee") :=``good\_func"$\\
Since this transformation removes the call to the sensitive API that causes the failure, the CPG rule for this feature is broken and the feature ``Sensitive Write API'' no longer remains. This also ensures that the sample does not contain a function call that causes failures. Therefore, the tools should change their predictions for this transformation.
